Symbolic Model Checking in External Memory

We extend the external memory BDD package Adiar with support for monotone variable substitution. Doing so, it now supports the relational product operation at the heart of symbolic model checking. We also identify additional avenues for merging variable substitution fully and the conjunction operation partially inside the relational product's existential quantification step. For smaller BDDs, these additional ideas improve the running of Adiar for model checking tasks up to 47%. For larger instances, the computation time is mostly unaffected as it is dominated by the existential quantification. Adiar's relational product is about one order of magnitude slower than conventional depth-first BDD implementations. Yet, its I/O-efficiency allows its running time to be virtually independent of the amount of internal memory. This allows it to compute on BDDs with much less internal memory and potentially to solve model checking tasks beyond the reach of conventional implementations. Compared to the only other external memory BDD package, CAL, Adiar is several orders of magnitude faster when computing on larger instances.

==> data/deadlock.adiar-exists_replace.tex <==
3.503      1.0936621916952858 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.013      1.0                % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
4.449      2.2560851926977685 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.024      0.96               % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.017      1.0                % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.015      1.0714285714285714 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.017      1.307692307692308  % bnet/davidich_yeast.bnet | async (disjoint)
0.012      1.090909090909091  % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.106      1.6825396825396826 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.016      1.0                % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.029      1.1153846153846154 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.017      1.0                % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.011      1.0                % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.028      1.0                % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.027      1.0                % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.016      2.0                % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.298      1.1417624521072796 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
36.19      0.9498438361197868 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/randomnet_n15k3.bnet | async (disjoint)
0.027      1.0384615384615385 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.022      1.0476190476190474 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
2.884      1.5881057268722465 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.14       1.1475409836065575 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
225.004    1.8497685775121466 % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
0.022      1.0476190476190474 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/dinwoodie_life.bnet | async (disjoint)
0.011      1.8333333333333333 % bnet/multivalued.bnet | async (disjoint)
0.018      1.0588235294117645 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.269      2.425568181818182  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.552      1.0415094339622641 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.015      1.3636363636363638 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.026      2.1666666666666665 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.261      1.6415094339622642 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.536      1.84192439862543   % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.02       0.9523809523809523 % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
9.906      1.811962685202122  % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.479      1.657439446366782  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.021      1.0                % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.015      1.0                % bnet/n12c5.bnet | async (disjoint)
0.015      1.153846153846154  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
62.716     2.065200210748156  % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
0.101      1.6833333333333336 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.018      1.2                % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.016      1.1428571428571428 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.016      0.888888888888889  % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.453      1.0942028985507248 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
9.027      1.0426195426195426 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.028      1.037037037037037  % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
18.772     1.5552609776304887 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.026      0.9629629629629629 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.182      1.205298013245033  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.027      1.0                % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
23.386     2.3807390817469205 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
1.069      1.9614678899082567 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
8.232      1.0538983484829085 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
2.073      2.1913319238900635 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.014      1.0                % bnet/faure_cellcycle.bnet | async (disjoint)
0.011      0.4583333333333333 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.036      3.2727272727272725 % bnet/arellano_rootstem.bnet | async (disjoint)
0.451      1.0789473684210527 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
0.079      1.1617647058823528 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.037      2.055555555555556  % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.21       1.7796610169491525 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.016      1.0                % bnet/tournier_apoptosis.bnet | async (disjoint)
0.018      0.9473684210526315 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.021      1.0                % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.012      0.9230769230769231 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.03       1.0                % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)


==> data/deadlock.adiar-pruning_and.tex <==
3.503      1.0488023952095809 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.013      1.0                % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
4.449      2.3514799154334036 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.024      0.96               % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.017      1.0                % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.015      1.0714285714285714 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.017      1.2142857142857144 % bnet/davidich_yeast.bnet | async (disjoint)
0.012      1.3333333333333335 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.106      1.6825396825396826 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.016      1.0                % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.029      1.16               % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.017      1.0                % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.011      1.0999999999999999 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.028      1.0                % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.027      1.0384615384615385 % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.016      2.0                % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.298      1.0915750915750915 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
36.19      1.0084712701331995 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/randomnet_n15k3.bnet | async (disjoint)
0.027      1.0384615384615385 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
2.884      1.5854865310610224 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.14       1.0852713178294575 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
225.004    1.847293147895765  % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
0.022      1.0                % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/dinwoodie_life.bnet | async (disjoint)
0.011      1.8333333333333333 % bnet/multivalued.bnet | async (disjoint)
0.018      1.0588235294117645 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.269      2.398314606741573  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.552      1.0203327171903882 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.015      1.3636363636363638 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.026      2.1666666666666665 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.261      1.6211180124223603 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.536      1.8231292517006805 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.02       0.9523809523809523 % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
9.906      1.7958665699782452 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.479      1.6460481099656359 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.021      1.0                % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.015      1.0                % bnet/n12c5.bnet | async (disjoint)
0.015      1.153846153846154  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
62.716     2.0405401008622093 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
0.101      1.6833333333333336 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.018      1.125              % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.016      1.1428571428571428 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.018      0.9473684210526315 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.016      0.9411764705882353 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.453      1.063380281690141  % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
9.027      1.0171267605633802 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.028      0.9655172413793103 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
18.772     1.6363319386331938 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.026      1.0                % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.182      1.205298013245033  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.027      1.0                % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
23.386     2.3617451019995963 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
1.069      1.950729927007299  % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
8.232      1.0274588117823265 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
2.073      2.175236096537251  % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.014      1.076923076923077  % bnet/faure_cellcycle.bnet | async (disjoint)
0.011      1.0                % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.036      3.2727272727272725 % bnet/arellano_rootstem.bnet | async (disjoint)
0.451      1.1446700507614214 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
0.079      1.1285714285714286 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.037      2.055555555555556  % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.21       1.75               % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.016      1.0                % bnet/tournier_apoptosis.bnet | async (disjoint)
0.018      1.0588235294117645 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.021      1.0                % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.03       0.5882352941176471 % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)


==> data/deadlock.adiar-shift_replace.tex <==
3.503      1.072894333843798  % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.013      1.0                % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
4.449      2.5050675675675675 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.024      0.96               % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.017      1.0                % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.015      1.0714285714285714 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.017      1.4166666666666667 % bnet/davidich_yeast.bnet | async (disjoint)
0.012      1.5                % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.106      1.7666666666666666 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.016      0.9411764705882353 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.029      1.16               % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.017      1.0                % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.011      1.0                % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.028      0.9655172413793103 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.027      1.0                % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.016      2.0                % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.298      1.1161048689138575 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
36.19      0.9495946052320853 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/randomnet_n15k3.bnet | async (disjoint)
0.027      1.0384615384615385 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
2.884      1.6954732510288064 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.14       1.1290322580645162 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
225.004    2.1792577095924375 % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
0.022      1.0                % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/dinwoodie_life.bnet | async (disjoint)
0.011      1.8333333333333333 % bnet/multivalued.bnet | async (disjoint)
0.018      1.0588235294117645 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.269      2.523049645390071  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.552      1.0317757009345794 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.015      1.5                % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.026      2.1666666666666665 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.261      1.9477611940298507 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.536      1.9350180505415162 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.02       1.0                % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
9.906      1.9519211822660099 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.479      1.7545787545787543 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.021      1.0                % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.015      1.0                % bnet/n12c5.bnet | async (disjoint)
0.015      1.153846153846154  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
62.716     2.3211813908730896 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
0.101      1.8035714285714286 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.018      1.2                % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.016      1.0666666666666667 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.016      0.9411764705882353 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.453      1.0785714285714287 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
9.027      1.0453966415749854 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.028      1.0                % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
18.772     1.7174748398902104 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.026      1.0                % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.182      1.2133333333333334 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.027      1.0                % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
23.386     2.550828970331588  % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
1.069      2.2224532224532223 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
8.232      1.0425531914893615 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
2.073      2.3033333333333332 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.014      1.0                % bnet/faure_cellcycle.bnet | async (disjoint)
0.011      1.0                % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.036      4.0                % bnet/arellano_rootstem.bnet | async (disjoint)
0.451      1.066193853427896  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
0.079      1.144927536231884  % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.037      1.9473684210526316 % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.21       1.8918918918918919 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.016      1.0                % bnet/tournier_apoptosis.bnet | async (disjoint)
0.018      0.9473684210526315 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.021      0.9545454545454547 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.03       1.0                % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)


==> data/deadlock.adiar-skip_transpose.tex <==
3.503      1.0257686676427527 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.013      0.9285714285714285 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
4.449      1.9616402116402119 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.024      0.96               % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.017      1.0                % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.015      1.0714285714285714 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.017      1.0                % bnet/davidich_yeast.bnet | async (disjoint)
0.012      1.2                % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.106      1.452054794520548  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.016      0.888888888888889  % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.029      1.1153846153846154 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.017      1.0                % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.011      1.0                % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.028      0.9655172413793103 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.027      1.0                % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.016      2.0                % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.298      1.068100358422939  % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
36.19      0.9207245713122678 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.018      1.0588235294117645 % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/randomnet_n15k3.bnet | async (disjoint)
0.027      1.0384615384615385 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
2.884      1.3772683858643744 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.14       1.0                % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
225.004    1.7217278188009335 % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
0.022      1.0                % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.022      1.0                % bnet/dinwoodie_life.bnet | async (disjoint)
0.011      1.375              % bnet/multivalued.bnet | async (disjoint)
0.018      1.0                % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.269      2.152798789712557  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.552      0.9403747870528111 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.015      1.153846153846154  % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.026      2.1666666666666665 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.261      1.6012269938650308 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.536      1.654320987654321  % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.02       1.0                % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
9.906      1.6306172839506172 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.479      1.1682926829268292 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.021      1.0                % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.015      1.0                % bnet/n12c5.bnet | async (disjoint)
0.015      1.0                % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
62.716     1.839394650398874  % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
0.101      1.402777777777778  % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.018      1.0                % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.016      1.0666666666666667 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.018      1.0                % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.018      1.0                % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.016      0.9411764705882353 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (dijoint)
0.453      1.0760095011876485 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
9.027      0.9886102288905924 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.028      1.0                % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
18.772     1.243837794858203  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.026      0.9629629629629629 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.182      1.0705882352941176 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.027      1.0                % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
23.386     2.111602708803612  % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
1.069      1.654798761609907  % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
8.232      1.01018529880967   % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
2.073      2.130524152106886  % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.014      0.7                % bnet/faure_cellcycle.bnet | async (disjoint)
0.011      1.0                % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.036      2.769230769230769  % bnet/arellano_rootstem.bnet | async (disjoint)
0.451      1.0226757369614512 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
0.079      1.0675675675675675 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.037      2.176470588235294  % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.21       1.5789473684210524 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.016      1.0                % bnet/tournier_apoptosis.bnet | async (disjoint)
0.018      0.9473684210526315 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.021      1.0                % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.012      1.0                % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.03       1.0                % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)


==> data/deadlock.buddy.tex <==
0.001      0.005      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.005      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.005      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.009      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.012      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.011      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.003      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.021      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.018      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.02       % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.013      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.014      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.025      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.026      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.018      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.004      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.026      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.028      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.029      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.011      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.002      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.03       % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.009      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.003      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.012      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.004      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.022      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.002      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.017      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.014      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.006      % bnet/multivalued.bnet | async (disjoint)
0.001      0.002      % bnet/multivalued.bnet | async (joint)
0.001      0.015      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.005      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.005      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.006      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.003      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.022      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.008      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.017      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.016      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.007      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
0.147      1.701      % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.045      0.535      % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.115      1.692      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.028      0.423      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
1.992      10.93      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.45       7.896      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.001      0.06       % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.013      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.003      0.134      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.002      0.025      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.008      0.277      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.007      0.069      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.026      0.481      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.031      0.267      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.019      0.9        % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.005      0.124      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.067      1.776      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.021      0.42       % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
0.58       9.168      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.303      8.635      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
1.623      27.019     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
1.167      38.111     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
4.246      103.248    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
%.???      155.355    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.001      0.111      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.015      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.122      5.075      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.211      3.265      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.003      0.056      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.001      0.015      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.065      0.273      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.021      0.15       % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/deadlock.cal.tex <==
0.001      0.008      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.012      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.01       %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.003      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.01       %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.011      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.008      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.008      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.012      %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.003      %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.012      %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.012      %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.019      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.018      %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.018      %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.022      %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.021      %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.017      %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.019      %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.018      %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.02       %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.013      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.014      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.025      %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.027      %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.003      %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.026      %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.022      %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.022      %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.027      %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.018      %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.004      %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.026      %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.028      %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.029      %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.011      %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.03       %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.002      %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.005      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.005      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.005      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.008      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.008      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.009      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.009      %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.003      %                    bnet/arellano_rootstem.bnet | async (joint)
0.001      0.012      %                    bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.004      %                    bnet/davidich_yeast.bnet | async (joint)
0.001      0.022      %                    bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.002      %                    bnet/dinwoodie_life.bnet | async (joint)
0.001      0.017      %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      %                    bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.014      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      %                    bnet/faure_cellcycle.bnet | async (joint)
0.001      0.006      %                    bnet/multivalued.bnet | async (disjoint)
0.001      0.002      %                    bnet/multivalued.bnet | async (joint)
0.001      0.015      %                    bnet/n12c5.bnet | async (disjoint)
0.001      0.001      %                    bnet/n12c5.bnet | async (joint)
0.001      0.002      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.002      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      %                    bnet/n3s1c1b.bnet | async (joint)
0.001      0.005      %                    bnet/n5s3.bnet | async (disjoint)
0.001      0.001      %                    bnet/n5s3.bnet | async (joint)
0.001      0.005      %                    bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      %                    bnet/n6s1c2.bnet | async (joint)
0.001      0.006      %                    bnet/n7s3.bnet | async (disjoint)
0.001      0.001      %                    bnet/n7s3.bnet | async (joint)
0.001      0.003      %                    bnet/raf.bnet | async (disjoint)
0.001      0.001      %                    bnet/raf.bnet | async (joint)
0.001      0.022      %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.008      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      %                    bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.017      %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      %                    bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.016      %                    bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      %                    bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.007      %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      %                    bnet/xiao_wnt5a.bnet | async (joint)
0.002      0.056      %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.001      0.015      %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.088      0.273      %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.03       0.15       %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.001      0.06       %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.013      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.004      0.134      %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.001      0.025      %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.014      0.277      %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.007      0.069      %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.04       0.481      %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.034      0.267      %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.027      0.9        %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.004      0.124      %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.077      1.776      %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.019      0.42       %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
0.641      9.168      %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
387.998    8.635      %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
19.353     27.019     %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
11677.955  38.111     %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
221.599    103.248    %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
20000      155.355    % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.001      0.111      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.015      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.162      5.075      %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
111.139    3.265      %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.152      1.701      %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.041      0.535      %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.126      1.692      %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.394      0.423      %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
1.97       10.93      %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
513.808    7.896      %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)


==> data/deadlock.cudd.tex <==
0.001      0.005      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.005      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.005      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.009      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.012      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.011      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.003      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.021      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.018      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.02       % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.013      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.014      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.025      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.026      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.018      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.004      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.026      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.028      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.029      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.011      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.002      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.03       % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.009      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.003      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.012      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.004      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.022      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.002      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.017      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.014      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.006      % bnet/multivalued.bnet | async (disjoint)
0.001      0.002      % bnet/multivalued.bnet | async (joint)
0.001      0.015      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.005      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.005      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.006      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.003      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.022      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.008      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.017      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.016      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.007      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
0.367      1.701      % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.034      0.535      % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.222      1.692      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.033      0.423      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
4.88       10.93      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.649      7.896      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.001      0.06       % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.013      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.003      0.134      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.001      0.025      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.015      0.277      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.005      0.069      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.063      0.481      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.023      0.267      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.025      0.9        % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.004      0.124      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.103      1.776      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.019      0.42       % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
2.133      9.168      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.481      8.635      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
9.237      27.019     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
2.129      38.111     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
51.733     103.248    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
10.882     155.355    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.001      0.111      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.015      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.793      5.075      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.484      3.265      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.002      0.056      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.001      0.015      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.103      0.273      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.02       0.15       % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/deadlock.libbdd.tex <==
0.001      0.005      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.005      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.005      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.009      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.012      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.011      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.003      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.021      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.018      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.02       % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.013      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.014      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.025      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.026      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.018      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.004      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.026      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.028      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.029      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.011      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.002      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.03       % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.009      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.003      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.012      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.004      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.022      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.002      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.017      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.014      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.006      % bnet/multivalued.bnet | async (disjoint)
0.001      0.002      % bnet/multivalued.bnet | async (joint)
0.001      0.015      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.005      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.005      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.006      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.003      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.022      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.008      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.017      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.016      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.007      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
0.363      1.701      % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.069      0.535      % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.277      1.692      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.05       0.423      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
5.039      10.93      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
2.042      7.896      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.002      0.06       % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.013      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.007      0.134      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.002      0.025      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.026      0.277      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.012      0.069      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.095      0.481      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.055      0.267      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.048      0.9        % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.008      0.124      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.17       1.776      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.032      0.42       % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
2.113      9.168      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.725      8.635      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
8.605      27.019     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
3.402      38.111     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
43.125     103.248    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
16.959     155.355    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.002      0.111      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.015      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.73       5.075      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.731      3.265      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.004      0.056      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.001      0.015      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.113      0.273      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.032      0.15       % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/deadlock.sylvan.tex <==
0.001      0.005      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.005      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.005      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.009      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.012      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.01       % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.011      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.008      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.003      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.012      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.018      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.021      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.017      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.019      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.018      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.02       % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.013      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.014      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.025      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.003      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.026      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.022      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.027      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.018      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.004      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.026      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.028      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.002      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.029      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.011      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.002      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.03       % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.002      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.009      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.003      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.012      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.004      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.022      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.002      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.017      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.014      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.006      % bnet/multivalued.bnet | async (disjoint)
0.001      0.002      % bnet/multivalued.bnet | async (joint)
0.001      0.015      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.002      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.005      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.005      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.006      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.003      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.022      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.008      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.017      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.016      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.007      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
0.06       1.701      % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.026      0.535      % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.046      1.692      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.027      0.423      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
1.725      10.93      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.779      7.896      % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.001      0.06       % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.013      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.001      0.134      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.001      0.025      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.003      0.277      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.004      0.069      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.017      0.481      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.026      0.267      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.007      0.9        % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.003      0.124      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.025      1.776      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.014      0.42       % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
0.265      9.168      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.335      8.635      % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.848      27.019     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
2.015      38.111     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
3.003      103.248    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
7.687      155.355    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.001      0.111      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.015      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.054      5.075      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.297      3.265      % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.001      0.056      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.001      0.015      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.031      0.273      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.027      0.15       % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/memory.gpufp_20_a.adiar.tex <==
1.0 1375.806
2.0 1241.758
4.0 1185.426
8.0 1114.898


==> data/memory.gpufp_20_a.buddy.tex <==
3.4501953125 510.151
3.5 491.476
4.0 445.494
8.0 341.295


==> data/memory.shield_s_ppp_010_a.adiar.tex <==
1.0 3483.432
2.0 3296.577
4.0 3259.706
8.0 3241.682
16.0 3132.347
32.0 3109.069
64.0 3120.579


==> data/memory.shield_s_ppp_010_a.buddy.tex <==
12.0 16836.731
16.0 5513.322
32.0 950.61
64.0 584.071


==> data/memory.smhome_16.adiar.tex <==
1.0 9619.21
2.0 9497.672
4.0 9515.419
8.0 9494.626


==> data/memory.smhome_16.buddy.tex <==
2.900390625 3527.894
3.0 2913.487
4.0 2072.352
8.0 1572.251


==> data/next.adiar-exists_replace.tex <==
1984.455   1.062405775935174  % 2020/SmartHome/smhome_16.pnml/states_23.bdd | next
1558.97    1.063076639822158  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
9683.261   1.0641203413708902 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | next
890.784    1.0580463087678789 % 2020/SmartHome/smhome_16.pnml/states_22.bdd | next
286.607    1.1567228332156192 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
571.012    1.1620365942257558 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
4131.401   1.0628524489283493 % 2020/SmartHome/smhome_16.pnml/states_24.bdd | next
358.795    1.0660401464191487 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
3265.815   1.061265043699235  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
169.709    1.1536981645139361 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
748.701    1.062226800086828  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
1272.263   1.1676733319811192 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next


==> data/next.adiar-pruning_and.tex <==
1984.455   1.0276447629320724 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | next
1558.97    1.0296606083502526 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
9683.261   1.0304612655762213 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | next
890.784    1.0231358275109947 % 2020/SmartHome/smhome_16.pnml/states_22.bdd | next
286.607    1.1346009200098177 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
571.012    1.1394329295182752 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
4131.401   1.0292650624711472 % 2020/SmartHome/smhome_16.pnml/states_24.bdd | next
358.795    1.024461208127277  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
3265.815   1.0274352712145471 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
169.709    1.1319593129898282 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
748.701    1.027092318835808  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
1272.263   1.1498717959146414 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next


==> data/next.adiar-shift_replace.tex <==
1984.455   1.0477979903153707 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | next
1558.97    1.0443386911149788 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
9683.261   1.0474655813039302 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | next
890.784    1.0456806789768391 % 2020/SmartHome/smhome_16.pnml/states_22.bdd | next
286.607    1.136058062009973  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
571.012    1.1444272973243812 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
4131.401   1.0479177351549251 % 2020/SmartHome/smhome_16.pnml/states_24.bdd | next
358.795    1.0386728655959427 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
3265.815   1.0432053966098056 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
169.709    1.1347142637452277 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
748.701    1.0423017756833701 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
1272.263   1.1487608678575072 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next


==> data/next.adiar-skip_transpose.tex <==
1984.455   1.0156930566886784 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | next
1558.97    1.0157433475349018 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
9683.261   1.0145562847726048 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | next
890.784    1.0153282208868666 % 2020/SmartHome/smhome_16.pnml/states_22.bdd | next
286.607    1.0861591983992238 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
571.012    1.0917781843976513 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
4131.401   1.0139823204761598 % 2020/SmartHome/smhome_16.pnml/states_24.bdd | next
358.795    1.016413551236399  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
3265.815   1.0160397777528196 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
169.709    1.084707521603518  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
748.701    1.0219471978728458 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
1272.263   1.1062329251899423 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next


==> data/next.buddy.tex <==
13.321     149.561    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
23.299     252.282    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
51.802     498.95     %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
183.092    1107.509   %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next
22.267     851.87     %  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
51.915     1893.929   %  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
149.432    3942.486   %  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
535.692    9244.467   %  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
18.313     345.436    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
46.519     718.315    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
143.532    1492.782   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
588.245    3130.558   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next


==> data/next.cal.tex <==
100000   149.561    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
100000   252.282    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
100000   498.95     %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
100000   1107.509   %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next
100000   851.87     %  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
100000   1893.929   %  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
100000   3942.486   %  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
100000   9244.467   %  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
100000   345.436    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
100000   718.315    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
100000   1492.782   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
100000   3130.558   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next


==> data/next.cudd.tex <==
214.494    345.436    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
587.529    718.315    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
1962.933   1492.782   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
4808.686   3130.558   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
54.777     851.87     %  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
151.371    1893.929   %  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
376.492    3942.486   %  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
1120.616   9244.467   %  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
35.077     149.561    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
73.229     252.282    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
160.782    498.95     %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
475.357    1107.509   %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next


==> data/next.libbdd.tex <==
37.829     149.561    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
63.184     252.282    %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
128.006    498.95     %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
282.063    1107.509   %  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next
67.382     851.87     %  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
156.991    1893.929   %  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
342.149    3942.486   %  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
858.073    9244.467   %  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
53.156     345.436    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
120.049    718.315    %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
268.183    1492.782   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
581.821    3130.558   %  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next


==> data/prev.adiar-exists_replace.tex <==
11586.811  1.0321927893560987 % 2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
32151.648  1.0280405017603693 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
6197.309   1.001442865499533  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
1969.104   1.0330256978457122 % 2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
16387.72   1.000211483524884  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
524.799    1.0929464417736254 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
2434.454   1.093391648656466  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev
1038.364   1.0995367257363413 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
311.903    1.091107853872014  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
4939.812   1.0338755735716276 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | prev


==> data/prev.adiar-pruning_and.tex <==
11586.811  1.0167655412037202 % 2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
32151.648  1.0139961511120588 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
6197.309   0.9842177272644256 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
1969.104   1.018825282503415  % 2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
16387.72   0.9820230031493228 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
524.799    1.077529725545593  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
2434.454   1.0808765810532899 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev
1038.364   1.0842256612450023 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
311.903    1.0744827443658238 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
4939.812   1.0176811314737488 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | prev


==> data/prev.adiar-shift_replace.tex <==
11586.811  1.024842237880846  % 2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
32151.648  1.0207930116949262 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
6197.309   0.9897968326483467 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
1969.104   1.0264587168014963 % 2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
16387.72   0.987525557812631  % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
524.799    1.0835387683807587 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
2434.454   1.0872913361631582 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev
1038.364   1.092617944009807  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
311.903    1.0808236219544736 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
4939.812   1.0260137619852419 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | prev


==> data/prev.adiar-skip_transpose.tex <==
11586.811  0.996103552787171  % 2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
32151.648  0.9949894097084574 % 2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
6197.309   0.9797954342259931 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
1969.104   0.99645666781033   % 2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
16387.72   0.9788422979151582 % 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
524.799    1.0430911971124126 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
2434.454   1.0456063944473795 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev
1038.364   1.049224523037966  % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
311.903    1.0410126328788611 % 2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
4939.812   0.9961911380384251 % 2020/SmartHome/smhome_16.pnml/states_23.bdd | prev


==> data/prev.buddy.tex <==
18.313     345.436    %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
154.038    6261.193   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
46.519     718.315    %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
1180.526   16594.73   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
143.532    1492.782   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
11220.856  100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | prev
588.245    3130.558   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
100000     100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | prev
22.267     851.87     %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
44.86      1918.347   %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
51.915     1893.929   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
133.732    4814.567   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | prev
149.432    3942.486   %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
423.031    11305.946  %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
535.692    9244.467   %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
2015.224   31496.736  %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
13.321     149.561    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
14.305     288.579    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
23.299     252.282    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
24.733     484.338    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
51.802     498.95     %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
55.507     950.345    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
183.092    1107.509   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next
206.417    2239.008   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev


==> data/prev.cal.tex <==
100000   345.436    %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
100000   6261.193   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
100000   718.315    %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
100000   16594.73   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
100000   1492.782   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
100000   100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | prev
100000   3130.558   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
100000   100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | prev
100000   851.87     %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
100000   1918.347   %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
100000   1893.929   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
100000   4814.567   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | prev
100000   3942.486   %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
100000   11305.946  %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
100000   9244.467   %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
100000   31496.736  %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
100000   149.561    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
100000   288.579    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
100000   252.282    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
100000   484.338    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
100000   498.95     %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
100000   950.345    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
100000   1107.509   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next
100000   2239.008   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev


==> data/prev.cudd.tex <==
699.202    6261.193   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
1707.56    16594.73   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
9624.394   100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | prev
100000     100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | prev
97.767     1918.347   %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
267.309    4814.567   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | prev
696.523    11305.946  %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
2639.762   31496.736  %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
37.632     288.579    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
69.822     484.338    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
170.816    950.345    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
503.657    2239.008   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev



==> data/prev.libbdd.tex <==
53.156     345.436    %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | next
287.335    6261.193   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_22.bdd | prev
120.049    718.315    %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | next
791.963    16594.73   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_23.bdd | prev
268.183    1492.782   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | next
2237.77    100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_24.bdd | prev
581.821    3130.558   %                  2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | next
18596.8615 100000     % ! NOTE ! TIMEOUT 2020/ShieldPPPs/shield_s_ppp_010_a.pnml/states_25.bdd | prev
67.382     851.87     %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | next
151.926    1918.347   %                  2020/SmartHome/smhome_16.pnml/states_22.bdd | prev
156.991    1893.929   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | next
386.93     4814.567   %                  2020/SmartHome/smhome_16.pnml/states_23.bdd | prev
342.149    3942.486   %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | next
932.901    11305.946  %                  2020/SmartHome/smhome_16.pnml/states_24.bdd | prev
858.073    9244.467   %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | next
3544.76    31496.736  %                  2020/SmartHome/smhome_16.pnml/states_25.bdd | prev
37.829     149.561    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | next
49.47      288.579    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_22.bdd | prev
63.184     252.282    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | next
85.419     484.338    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_23.bdd | prev
128.006    498.95     %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | next
174.876    950.345    %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_24.bdd | prev
282.063    1107.509   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | next
410.181    2239.008   %                  2021/GPUForwardProgress/gpufp_20_a.pnml/states_25.bdd | prev


==> data/reachability.adiar-exists_replace.tex <==
1517.381   1.1285016041969422 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.106      1.2325581395348837 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.974      1.0882681564245809 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.84       1.278538812785388  % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
2.64       1.3421453990849008 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
215.507    1.1038847284685442 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
30.82      1.0616237814749752 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
4.919      1.1044005388414908 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
45.688     1.125902560437665  % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
22.076     1.1590885225244147 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.334      1.1928571428571428 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
165.907    1.5049209473617373 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
818.237    1.1682991464462866 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
7.054      1.1698175787728027 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
868.354    1.0902929407200281 % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
11.961     1.0886502229908073 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
83.49      1.3626793321255446 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
19.352     1.1400966183574879 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
2.02       1.2515489467162328 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.602      1.162162162162162  % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
161.401    1.0526518313680477 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.183      1.1883116883116882 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
66.42      1.0887810635368174 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
1.786      1.1567357512953367 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
6.381      1.213348545350827  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
17.35      1.5113240418118468 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.951      1.3762662807525325 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
10.177     1.0692372347131749 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
10.461     1.4882629107981222 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
17.497     1.2158293377805574 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
23.309     1.0681422417743562 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)


==> data/reachability.adiar-pruning_and.tex <==
1517.381   1.150398216837692  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.106      1.2045454545454546 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.974      1.0507011866235167 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.84       1.2                % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
2.64       1.196193928409606  % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
215.507    1.057277561913733  % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
30.82      1.0160551214848514 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
4.919      1.068883094306823  % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
45.688     1.0955041361947009 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
22.076     1.1572050112701158 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.334      1.1517241379310346 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
165.907    1.4826362823949955 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
818.237    1.0211203362481327 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
7.054      1.1494215414697737 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
868.354    1.069159205303232  % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
11.961     1.0337049520352606 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
83.49      1.3199999999999998 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
19.352     1.1031180527845865 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
2.02       1.1444759206798867 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.602      1.1532567049808429 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
161.401    1.0078428923787817 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.183      1.1582278481012658 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
66.42      1.1438116723208596 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
1.786      1.1225644248900064 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
6.381      1.1904850746268656 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
17.35      1.534990710430859  % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.951      1.2596026490066226 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
10.177     1.0405930470347649 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
10.461     1.4345858475041142 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
17.497     1.1761107750218458 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
23.309     1.1447303801198312 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)


==> data/reachability.adiar-shift_replace.tex <==
1517.381   1.1114341298198274 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.106      1.2325581395348837 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.974      1.095613048368954  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.84       1.2844036697247705 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
2.64       1.3082259663032707 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
215.507    1.1043938586421778 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
30.82      1.0313211082853702 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
4.919      1.1368153455049688 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
45.688     1.2066342700190156 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
22.076     1.1218619778432768 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.334      1.1719298245614036 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
165.907    1.5173634293344553 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
818.237    1.141235050036612  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
7.054      1.1393958972702312 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
868.354    1.1008586493102788 % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
11.961     1.082051745974308  % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
83.49      1.3539504411001555 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
19.352     1.1278703811633057 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
2.02       1.2227602905569008 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.602      1.1466666666666665 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
161.401    1.046366589086477  % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.183      1.1806451612903226 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
66.42      1.04248740445435   % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
1.786      1.152258064516129  % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
6.381      1.2001128455896182 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
17.35      1.5818745441283737 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.951      1.3413258110014104 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
10.177     0.9994107826770107 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
10.461     1.5141120277898394 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
17.497     1.2409219858156029 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
23.309     1.0401624347360436 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)


==> data/reachability.adiar-skip_transpose.tex <==
1517.381   1.054457351412354  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
0.106      1.2045454545454546 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.974      1.103057757644394  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.84       1.2650602409638554 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
2.64       1.213793103448276  % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
215.507    1.0073527349556406 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
30.82      0.9870928482208629 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
4.919      1.1447521526646498 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
45.688     1.1021904853806814 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
22.076     1.064057454089748  % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.334      1.1245791245791248 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
165.907    1.4866884717057216 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
818.237    1.011050372299807  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
7.054      1.1219977731827582 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
868.354    1.0393996921375375 % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
11.961     1.1089375115890971 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
83.49      1.2546585717720606 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
19.352     1.0930863081789426 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
2.02       1.1074561403508771 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.602      1.1510516252390057 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
161.401    1.0132016723373802 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.183      1.1226993865030674 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
66.42      0.9801086058316609 % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
1.786      1.1582360570687418 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
6.381      1.1062760055478502 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
17.35      1.4154021863272968 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.951      1.2114649681528662 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
10.177     1.0024625689519306 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
10.461     1.5683658170914543 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
17.497     1.066760151201073  % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
23.309     1.0369233506828597 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)


==> data/reachability.buddy.tex <==
0.001      0.001      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.001      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.001      %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.001      %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.001      %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.001      %                    bnet/arellano_rootstem.bnet | async (joint)
0.001      0.001      %                    bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.001      %                    bnet/davidich_yeast.bnet | async (joint)
0.001      0.001      %                    bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.001      %                    bnet/dinwoodie_life.bnet | async (joint)
0.001      0.001      %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      %                    bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.001      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      %                    bnet/faure_cellcycle.bnet | async (joint)
0.001      0.001      %                    bnet/multivalued.bnet | async (disjoint)
0.001      0.001      %                    bnet/multivalued.bnet | async (joint)
0.001      0.001      %                    bnet/n12c5.bnet | async (disjoint)
0.001      0.001      %                    bnet/n12c5.bnet | async (joint)
0.001      0.001      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.001      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      %                    bnet/n3s1c1b.bnet | async (joint)
0.001      0.001      %                    bnet/n5s3.bnet | async (disjoint)
0.001      0.001      %                    bnet/n5s3.bnet | async (joint)
0.001      0.001      %                    bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      %                    bnet/n6s1c2.bnet | async (joint)
0.001      0.001      %                    bnet/n7s3.bnet | async (disjoint)
0.001      0.001      %                    bnet/n7s3.bnet | async (joint)
0.001      0.001      %                    bnet/raf.bnet | async (disjoint)
0.001      0.001      %                    bnet/raf.bnet | async (joint)
0.001      0.001      %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.001      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      %                    bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.001      %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      %                    bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.001      %                    bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      %                    bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.001      %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      %                    bnet/xiao_wnt5a.bnet | async (joint)
0.992      154.249    %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.131      29.884     %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.752      109.339    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.248      22.409     %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
21.876     1365.246   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
6.545      716.975    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.002      0.889      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.155      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.012      4.327      %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.006      0.525      %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.033      11.054     %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.02       1.652      %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.126      37.864     %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.068      6.191      %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.035      6.909      %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.01       0.709      %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.109      10.968     %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.038      2.018      %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
0.861      61.664     %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.429      19.678     %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
2.492      195.136    %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
1.397      63.713     %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
7.143      788.797    %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
20000      195.269    % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.002      0.654      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.086      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.186      14.1       %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.154      10.183     %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.01       1.55       %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.007      0.285      %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.355      17.158     %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.195      5.317      %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/reachability.cal.tex <==
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.001      % bnet/multivalued.bnet | async (disjoint)
0.001      0.001      % bnet/multivalued.bnet | async (joint)
0.001      0.001      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.001      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.001      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.001      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.001      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
0.033      1.55       % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.008      0.285      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
1.375      17.158     % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.822      5.317      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.012      0.889      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.003      0.155      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.078      4.327      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.01       0.525      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.252      11.054     % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.046      1.652      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
1.065      37.864     % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.217      6.191      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.195      6.909      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.025      0.709      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.522      10.968     % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.066      2.018      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
4.702      61.664     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
74.248     19.678     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
24.222     195.136    % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
650.307    63.713     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
1303.764   788.797    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
7560.6     195.269    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.012      0.654      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.002      0.086      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.962      14.1       % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
21.678     10.183     % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
5.931      154.249    % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
1.181      29.884     % mcc/2023/Anderson/anderson_04.pnml | async (joint)
3.986      109.339    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
10.897     22.409     % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
83.009     1365.246   % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
800.03     716.975    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)


==> data/reachability.cudd.tex <==
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.001      % bnet/multivalued.bnet | async (disjoint)
0.001      0.001      % bnet/multivalued.bnet | async (joint)
0.001      0.001      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.001      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.001      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.001      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.001      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
2.345      154.249    % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.234      29.884     % mcc/2023/Anderson/anderson_04.pnml | async (joint)
1.286      109.339    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.488      22.409     % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
57.855     1365.246   % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
20.119     716.975    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.001      0.889      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.155      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.014      4.327      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.004      0.525      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.058      11.054     % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.024      1.652      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.373      37.864     % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.107      6.191      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.037      6.909      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.013      0.709      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.109      10.968     % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.052      2.018      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
1.894      61.664     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.865      19.678     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
6.424      195.136    % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
3.095      63.713     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
21.402     788.797    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
11.44      195.269    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.001      0.654      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.086      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.221      14.1       % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.262      10.183     % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.008      1.55       % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.003      0.285      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.856      17.158     % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.292      5.317      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/reachability.libbdd.tex <==
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.001      % bnet/multivalued.bnet | async (disjoint)
0.001      0.001      % bnet/multivalued.bnet | async (joint)
0.001      0.001      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.001      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.001      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.001      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.001      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
12.534     154.249    % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
3.496      29.884     % mcc/2023/Anderson/anderson_04.pnml | async (joint)
5.886      109.339    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
2.617      22.409     % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
177.907    1365.246   % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
187.149    716.975    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.013      0.889      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.005      0.155      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.078      4.327      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.037      0.525      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.287      11.054     % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.229      1.652      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
1.761      37.864     % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
1.161      6.191      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.241      6.909      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.055      0.709      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.634      10.968     % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.243      2.018      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
12.019     61.664     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
5.657      19.678     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
58.899     195.136    % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
23.056     63.713     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
292.048    788.797    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
97.467     195.269    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.009      0.654      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.002      0.086      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
2.129      14.1       % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
6.838      10.183     % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.033      1.55       % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.022      0.285      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
1.707      17.158     % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
1.176      5.317      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/reachability.sylvan.tex <==
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
0.001      0.001      % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
0.001      0.001      % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (disjoint)
0.001      0.001      % bnet/arellano_rootstem.bnet | async (joint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (disjoint)
0.001      0.001      % bnet/davidich_yeast.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_life.bnet | async (joint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.001      0.001      % bnet/dinwoodie_stomatal.bnet | async (joint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (disjoint)
0.001      0.001      % bnet/faure_cellcycle.bnet | async (joint)
0.001      0.001      % bnet/multivalued.bnet | async (disjoint)
0.001      0.001      % bnet/multivalued.bnet | async (joint)
0.001      0.001      % bnet/n12c5.bnet | async (disjoint)
0.001      0.001      % bnet/n12c5.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1a.bnet | async (joint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.001      % bnet/n3s1c1b.bnet | async (joint)
0.001      0.001      % bnet/n5s3.bnet | async (disjoint)
0.001      0.001      % bnet/n5s3.bnet | async (joint)
0.001      0.001      % bnet/n6s1c2.bnet | async (disjoint)
0.001      0.001      % bnet/n6s1c2.bnet | async (joint)
0.001      0.001      % bnet/n7s3.bnet | async (disjoint)
0.001      0.001      % bnet/n7s3.bnet | async (joint)
0.001      0.001      % bnet/raf.bnet | async (disjoint)
0.001      0.001      % bnet/raf.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n15k3.bnet | async (joint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      0.001      % bnet/randomnet_n7k3.bnet | async (joint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (disjoint)
0.001      0.001      % bnet/saadatpour_guardcell.bnet | async (joint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (disjoint)
0.001      0.001      % bnet/tournier_apoptosis.bnet | async (joint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (disjoint)
0.001      0.001      % bnet/xiao_wnt5a.bnet | async (joint)
0.958      154.249    % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.149      29.884     % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.694      109.339    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.388      22.409     % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
27.209     1365.246   % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
12.776     716.975    % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.001      0.889      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.001      0.155      % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.003      4.327      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.003      0.525      % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
0.018      11.054     % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.017      1.652      % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.112      37.864     % mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
0.077      6.191      % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.03       6.909      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.008      0.709      % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
0.089      10.968     % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
0.033      2.018      % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
1.068      61.664     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
0.551      19.678     % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
3.314      195.136    % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
2.583      63.713     % mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
11.294     788.797    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
8.633      195.269    % mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.001      0.654      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.086      % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
0.147      14.1       % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.27       10.183     % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.002      1.55       % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.002      0.285      % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
0.256      17.158     % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.319      5.317      % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/scc.adiar-exists_replace.tex <==
101.424    1.28316591179373   % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
2.473      1.2352647352647352 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
27985.073  1.3051014152327067 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
2331.835   1.5362891643102417 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
4084.048   1.2746573384319027 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
91.88      1.4662560043406796 % bnet/faure_cellcycle.bnet | async (disjoint)
0.736      1.245346869712352  % bnet/n7s3.bnet | async (joint)
6.046      1.4310059171597636 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
27822.061  1.6802465056692646 % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
337.706    1.691481635453867  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
173.02     1.4710958822579137 % bnet/saadatpour_guardcell.bnet | async (disjoint)
374.743    1.4731506160027046 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
6431.27    1.2874990115441634 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
265.491    4.2579387990762125 % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
34.3       1.380115076650706  % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
1.315      1.3769633507853403 % bnet/n6s1c2.bnet | async (disjoint)
2216.942   1.307474502990403  % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
6303.276   1.2793480096384289 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
14276.38   1.9185041763579276 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
59.932     1.4898451288935295 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
2853.436   1.2757906860496415 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
785.574    1.2642327449692943 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
782.452    1.5457338092970974 % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
93.326     1.472785519276595  % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
1276.115   1.2776494569978545 % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.107      1.244186046511628  % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
26.46      1.3064731150940603 % bnet/saadatpour_guardcell.bnet | async (joint)
106212.906 1.605521797842568  % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
19.097     1.3749730002159983 % bnet/xiao_wnt5a.bnet | async (disjoint)
0.868      1.215686274509804  % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.123      1.2436323366555924 % bnet/multivalued.bnet | async (joint)
75240.404  1.6494954180271164 % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
30.005     1.2483358295889497 % bnet/n12c5.bnet | async (joint)
378.681    1.269191323350002  % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.542      1.400516795865633  % bnet/raf.bnet | async (disjoint)
9649.283   1.5339136143756666 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
4.716      1.2586068855084067 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
7539.366   1.50436081836129   % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
173.719    1.483142518078358  % bnet/dinwoodie_stomatal.bnet | async (disjoint)
4837.777   1.4135499006408019 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.232      1.2210526315789474 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
9.495      1.267690253671562  % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
11884.195  1.562499342614564  % bnet/dinwoodie_life.bnet | async (disjoint)
17.139     1.4628712871287128 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
823.633    1.2551745683414863 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
10291.597  1.5502327775001983 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
48270.546  1.819892752335531  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.334      1.31496062992126   % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
10.405     1.453212290502793  % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
3270.277   1.298365270281269  % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
17.241     1.2534351145038167 % bnet/davidich_yeast.bnet | async (joint)
1435.649   1.0790304990834265 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.286      1.336448598130841  % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
770.567    1.543804782273333  % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
1148.263   1.7550534114061513 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
10.04      2.9093016516951606 % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
2.605      1.3638743455497382 % bnet/n7s3.bnet | async (disjoint)
2752.069   1.489359894362005  % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.039      1.21875            % bnet/n3s1c1a.bnet | async (joint)
22.831     1.2866884580703337 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
4140.611   1.2145385801088524 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
16446.601  1.5573421082683454 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
481.022    1.4952920659887905 % bnet/tournier_apoptosis.bnet | async (disjoint)
98.276     1.292986172326233  % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
36.024     1.4907510862818125 % bnet/randomnet_n15k3.bnet | async (disjoint)
80.338     1.2797158240147821 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
82.426     1.4571135624381277 % bnet/davidich_yeast.bnet | async (disjoint)
218.442    1.4785068868658837 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
65178.081  1.936153848141836  % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
4.707      1.4088596228674048 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
211.962    1.0306377971516232 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
4.654      1.2487255165012074 % bnet/xiao_wnt5a.bnet | async (joint)
168.787    1.4553363568952733 % bnet/n12c5.bnet | async (disjoint)
604.915    2.064042064605064  % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
1575.205   1.3025274011965153 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
1537.788   1.256694372779745  % bnet/dinwoodie_life.bnet | async (joint)
0.259      1.251207729468599  % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.837      1.3676470588235294 % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
2249.329   1.4690675561204265 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
1947.618   1.4597055733016353 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
1052.287   1.275505578208864  % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
175.68     1.2895553940675166 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.077      1.3275862068965516 % bnet/n3s1c1b.bnet | async (disjoint)
15.612     1.099359200056334  % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.511      1.2283653846153848 % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
1.639      1.214074074074074  % bnet/randomnet_n7k3.bnet | async (joint)
141.604    1.2789840673434736 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
17907.949  1.5730414467033191 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
19.976     0.47534742052160667 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
3.76       1.5027977617905677 % bnet/multivalued.bnet | async (disjoint)
6.4        1.3640238704177323 % bnet/randomnet_n7k3.bnet | async (disjoint)
4243.465   1.521483080868201  % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.174      1.264848484848485  % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
6.28       1.2612974492870055 % bnet/randomnet_n15k3.bnet | async (joint)
17.11      1.360527989821883  % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
25.603     1.2662215628091    % bnet/dinwoodie_stomatal.bnet | async (joint)
1.366      1.2683379758588673 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
34823.789  1.5832619950304074 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
355.76     1.2734184283433676 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
18160.492  1.5694840417786022 % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
19.315     1.2703058204537983 % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
40.358     1.2517990074441685 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
44.156     1.1019440493124704 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
23.536     1.581720430107527  % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
126.005    4.108680057388809  % bnet/arellano_rootstem.bnet | async (disjoint)
0.042      1.2                % bnet/n3s1c1b.bnet | async (joint)
0.192      1.2307692307692308 % bnet/n5s3.bnet | async (joint)
0.074      1.3214285714285714 % bnet/n3s1c1a.bnet | async (disjoint)
18.975     1.2613001861207127 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
420.506    1.399643187612752  % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.689      1.3807615230460921 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2407.238   1.5166617838387848 % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2.37       1.371527777777778  % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
13479.298  1.52245798960473   % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
4.188      1.2390532544378698 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
6.161      1.393576114001357  % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
51.626     1.531292638073204  % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
644.269    4.360239577693558  % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
4159.577   1.5205683263383734 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2027.243   1.2104048907153906 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
40933.506  1.609638616944563  % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
55999.634  1.6909911495360495 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
6308.131   1.3236436711086565 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
2.644      1.26810551558753   % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
519.891    1.3797129064703524 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.397      1.2177914110429449 % bnet/n6s1c2.bnet | async (joint)
17.555     0.4707191505335979 % bnet/faure_cellcycle.bnet | async (joint)
0.579      1.3985507246376812 % bnet/n5s3.bnet | async (disjoint)
20178.386  1.3787245108586996 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
3.821      1.24828487422411   % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
22.566     1.3891898547155872 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
771.909    1.2766486338083842 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
3251.146   1.3035028612828121 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.216      1.2485549132947977 % bnet/raf.bnet | async (joint)
3391.882   1.29544607365356   % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
155.056    1.8152401690490407 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
4167.131   1.5404270844923755 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2703.455   1.5339535068457395 % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
15637.631  1.5955333602696902 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
77.479     1.1849478481632154 % bnet/tournier_apoptosis.bnet | async (joint)
9.383      1.2726163027261628 % bnet/arellano_rootstem.bnet | async (joint)
837.529    1.5010394898613895 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)


==> data/scc.adiar-pruning_and.tex <==
101.424    1.2658379511756779 % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
2.473      1.2098825831702542 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
27985.073  1.273489494546808  % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
2331.835   1.4347378803139665 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
4084.048   1.2654117218382583 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
91.88      1.3892374918729304 % bnet/faure_cellcycle.bnet | async (disjoint)
0.736      1.2105263157894737 % bnet/n7s3.bnet | async (joint)
6.046      1.3411712511091394 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
27822.061  1.5648699668015664 % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
337.706    1.928194997173706  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
173.02     1.398695240943889  % bnet/saadatpour_guardcell.bnet | async (disjoint)
374.743    1.4021087211107826 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
6431.27    1.2682991956074634 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
265.491    3.9867105144607624 % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
34.3       1.3697536040892935 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
1.315      1.2804284323271666 % bnet/n6s1c2.bnet | async (disjoint)
2216.942   1.2805648264636194 % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
6303.276   1.2626828160660388 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
14276.38   1.8634063926869118 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
59.932     1.4609365477902638 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
2853.436   1.2535181444615968 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
785.574    1.241274370849312  % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
782.452    1.4551669499689421 % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
93.326     1.4074196953702305 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
1276.115   1.2569044720492    % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.107      1.202247191011236  % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
26.46      1.3380530973451328 % bnet/saadatpour_guardcell.bnet | async (joint)
106212.906 1.5567222877120752 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
19.097     1.2902506587392744 % bnet/xiao_wnt5a.bnet | async (disjoint)
0.868      1.1988950276243093 % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.123      1.2646396396396395 % bnet/multivalued.bnet | async (joint)
75240.404  1.5377565752178532 % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
30.005     1.2149740848720438 % bnet/n12c5.bnet | async (joint)
378.681    1.2336814876593083 % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.542      1.3155339805825244 % bnet/raf.bnet | async (disjoint)
9649.283   1.51227415289115   % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
4.716      1.2303678580746151 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
7539.366   1.4271774473371721 % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
173.719    1.3987938031435196 % bnet/dinwoodie_stomatal.bnet | async (disjoint)
4837.777   1.3932056351689188 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.232      1.1958762886597938 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
9.495      1.2408520648196548 % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
11884.195  1.468816767867602  % bnet/dinwoodie_life.bnet | async (disjoint)
17.139     1.3806186563557274 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
823.633    1.2257118323479121 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
10291.597  1.4537597447882185 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
48270.546  1.7967017886192904 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.334      1.2796934865900382 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
10.405     1.3819896400584406 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
3270.277   1.2745607912052623 % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
17.241     1.2322041166380788 % bnet/davidich_yeast.bnet | async (joint)
1435.649   1.0214558165711247 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.286      1.2825112107623318 % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
770.567    1.4727652897205907 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
1148.263   1.7585933862628342 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
10.04      2.76355628956785   % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
2.605      1.2870553359683794 % bnet/n7s3.bnet | async (disjoint)
2752.069   1.4778502543481915 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.039      1.21875            % bnet/n3s1c1a.bnet | async (joint)
22.831     1.2683888888888888 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
4140.611   1.2547922049506672 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
16446.601  1.4741969389167315 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
481.022    1.4135192079952748 % bnet/tournier_apoptosis.bnet | async (disjoint)
98.276     1.2576752281132824 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
36.024     1.417263356676371  % bnet/randomnet_n15k3.bnet | async (disjoint)
80.338     1.2608170247492898 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
82.426     1.373675088327445  % bnet/davidich_yeast.bnet | async (disjoint)
218.442    1.4891911238367932 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
65178.081  1.6919839446296359 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
4.707      1.3799472295514512 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
211.962    0.9244719315768125 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
4.654      1.217687074829932  % bnet/xiao_wnt5a.bnet | async (joint)
168.787    1.441035098054282  % bnet/n12c5.bnet | async (disjoint)
604.915    2.0458919143783842 % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
1575.205   1.273125435433057  % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
1537.788   1.273426029667133  % bnet/dinwoodie_life.bnet | async (joint)
0.259      1.227488151658768  % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.837      1.3078124999999998 % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
2249.329   1.445984716846376  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
1947.618   1.3873840117509113 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
1052.287   1.4137086969080197 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
175.68     1.2616339193381594 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.077      1.2622950819672132 % bnet/n3s1c1b.bnet | async (disjoint)
15.612     1.0358967553579723 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.511      1.2023529411764706 % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
1.639      1.194606413994169  % bnet/randomnet_n7k3.bnet | async (joint)
141.604    1.245231583668229  % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
17907.949  1.4833354966061192 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
19.976     1.336544894955172  % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
3.76       1.4630350194552528 % bnet/multivalued.bnet | async (disjoint)
6.4        1.3496415014761705 % bnet/randomnet_n7k3.bnet | async (disjoint)
4243.465   1.4425880246018785 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.174      1.2244059841595778 % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
6.28       1.2549960031974423 % bnet/randomnet_n15k3.bnet | async (joint)
17.11      1.2883066034184172 % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
25.603     1.2626621295063372 % bnet/dinwoodie_stomatal.bnet | async (joint)
1.366      1.2440801457194899 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
34823.789  1.5128851029266839 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
355.76     1.2356939663706177 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
18160.492  1.48505434693724   % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
19.315     1.2364765379937264 % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
40.358     1.2205655526992287 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
44.156     1.1510948905109488 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
23.536     1.4704485817818318 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
126.005    3.8600925160064943 % bnet/arellano_rootstem.bnet | async (disjoint)
0.042      1.1666666666666667 % bnet/n3s1c1b.bnet | async (joint)
0.192      1.1851851851851851 % bnet/n5s3.bnet | async (joint)
0.074      1.2758620689655171 % bnet/n3s1c1a.bnet | async (disjoint)
18.975     1.2472885032537964 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
420.506    1.3954119642009761 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.689      1.33011583011583   % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2407.238   1.414998559865509  % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2.37       1.286644951140065  % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
13479.298  1.4334056418509038 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
4.188      1.2177958708927012 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
6.161      1.3570484581497797 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
51.626     1.433299092145812  % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
644.269    4.121264264878972  % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
4159.577   1.4379844184075194 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2027.243   1.2410509039240545 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
40933.506  1.5226330449877767 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
55999.634  1.6130384710461445 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
6308.131   1.2897104181821677 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
2.644      1.2518939393939394 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
519.891    1.382516015285323  % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.397      1.188622754491018  % bnet/n6s1c2.bnet | async (joint)
17.555     1.2706282570932252 % bnet/faure_cellcycle.bnet | async (joint)
0.579      1.3591549295774648 % bnet/n5s3.bnet | async (disjoint)
20178.386  1.3328296181864285 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
3.821      1.2219379597057884 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
22.566     1.3473847623596846 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
771.909    1.2345013433981578 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
3251.146   1.2699699767736008 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.216      1.2134831460674158 % bnet/raf.bnet | async (joint)
3391.882   1.2683811348666623 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
155.056    1.6338883034773446 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
4167.131   1.456207856216313  % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2703.455   1.438060758612949  % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
15637.631  1.4939011132204676 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
77.479     1.2357688565641098 % bnet/tournier_apoptosis.bnet | async (joint)
9.383      1.2260551417744674 % bnet/arellano_rootstem.bnet | async (joint)
837.529    1.4044276086653955 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)


==> data/scc.adiar-shift_replace.tex <==
101.424    1.3088487695345268 % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
2.473      1.2471003530005043 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
27985.073  1.3047231320397346 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
2331.835   1.6079668950527386 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
4084.048   1.2956109000075502 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
91.88      1.5084550976851092 % bnet/faure_cellcycle.bnet | async (disjoint)
0.736      1.2689655172413794 % bnet/n7s3.bnet | async (joint)
6.046      1.4884293451501722 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
27822.061  1.7675584424808763 % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
337.706    1.6601579014639807 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
173.02     1.5438978468237752 % bnet/saadatpour_guardcell.bnet | async (disjoint)
374.743    1.5433780739435026 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
6431.27    0.5376723534981681 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
265.491    4.410149501661129  % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
34.3       1.3997714658831208 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
1.315      1.4514348785871964 % bnet/n6s1c2.bnet | async (disjoint)
2216.942   1.3267077994745693 % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
6303.276   1.3046881646182322 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
14276.38   1.983111496350872  % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
59.932     1.54031201007479   % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
2853.436   1.3131024657060195 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
785.574    1.2694401577157075 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
782.452    1.6353072476247403 % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
93.326     1.5664244112858556 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
1276.115   1.3051146474667104 % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.107      1.2738095238095237 % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
26.46      1.3308520269590585 % bnet/saadatpour_guardcell.bnet | async (joint)
106212.906 1.6517476048798763 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
19.097     1.4297372164408177 % bnet/xiao_wnt5a.bnet | async (disjoint)
0.868      1.215686274509804  % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.123      1.2732426303854876 % bnet/multivalued.bnet | async (joint)
75240.404  1.702308942074068  % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
30.005     1.2802952722307561 % bnet/n12c5.bnet | async (joint)
378.681    1.2797773542055315 % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.542      1.4808743169398908 % bnet/raf.bnet | async (disjoint)
9649.283   1.6044783403439558 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
4.716      1.2881726304288446 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
7539.366   1.5741686844793752 % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
173.719    1.531981127915693  % bnet/dinwoodie_stomatal.bnet | async (disjoint)
4837.777   1.3953949267931927 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.232      1.2473118279569892 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
9.495      1.2950081833060556 % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
11884.195  1.660302557374429  % bnet/dinwoodie_life.bnet | async (disjoint)
17.139     1.5279486493714896 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
823.633    1.271970966371955  % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
10291.597  1.6103419231508858 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
48270.546  1.919284941445573  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.334      1.2996108949416343 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
10.405     1.5161008305405796 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
3270.277   1.322130673663528  % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
17.241     1.297877145438121  % bnet/davidich_yeast.bnet | async (joint)
1435.649   1.0624693799315885 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.286      1.395121951219512  % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
770.567    1.619767219434676  % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
1148.263   1.827949440438098  % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
10.04      2.9203025014543336 % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
2.605      1.4180729450190528 % bnet/n7s3.bnet | async (disjoint)
2752.069   1.5747110717951829 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.039      1.3                % bnet/n3s1c1a.bnet | async (joint)
22.831     1.3852921546022692 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
4140.611   1.2180585540836741 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
16446.601  1.624434108472004  % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
481.022    1.548721316964645  % bnet/tournier_apoptosis.bnet | async (disjoint)
98.276     1.3000330709703023 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
36.024     1.5370567905448649 % bnet/randomnet_n15k3.bnet | async (disjoint)
80.338     1.300304285899262  % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
82.426     1.6093484585196323 % bnet/davidich_yeast.bnet | async (disjoint)
218.442    1.4645498246766744 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
65178.081  1.912424488110637  % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
4.707      1.4590824550526968 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
211.962    0.8823808572284942 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
4.654      1.275417922718553  % bnet/xiao_wnt5a.bnet | async (joint)
168.787    1.5145454219159398 % bnet/n12c5.bnet | async (disjoint)
604.915    2.1043522728458663 % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
1575.205   1.3244986058838761 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
1537.788   1.2629250024637824 % bnet/dinwoodie_life.bnet | async (joint)
0.259      1.2634146341463415 % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.837      1.4307692307692308 % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
2249.329   1.465321773164365  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
1947.618   1.5174273470977795 % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
1052.287   1.5869683899378657 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
175.68     1.3036896316305027 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.077      1.375              % bnet/n3s1c1b.bnet | async (disjoint)
15.612     1.0845432441820078 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.511      1.2463414634146341 % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
1.639      1.2435508345978756 % bnet/randomnet_n7k3.bnet | async (joint)
141.604    1.2987498968183362 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
17907.949  1.6406992983031248 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
19.976     1.487526993819346  % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
3.76       1.5608136156081363 % bnet/multivalued.bnet | async (disjoint)
6.4        1.41749723145072   % bnet/randomnet_n7k3.bnet | async (disjoint)
4243.465   1.5939105990388756 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.174      1.2776247321701868 % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
6.28       1.285568065506653  % bnet/randomnet_n15k3.bnet | async (joint)
17.11      1.4112504124051468 % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
25.603     1.2824584251652977 % bnet/dinwoodie_stomatal.bnet | async (joint)
1.366      1.2802249297094659 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
34823.789  1.6958984468974667 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
355.76     1.2990579128021615 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
18160.492  1.6594875063896761 % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
19.315     1.30524395188539   % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
40.358     0.5099763700923714 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
44.156     1.0879613659882719 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
23.536     1.587267332074454  % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
126.005    4.357170026626093  % bnet/arellano_rootstem.bnet | async (disjoint)
0.042      1.2352941176470589 % bnet/n3s1c1b.bnet | async (joint)
0.192      1.2631578947368423 % bnet/n5s3.bnet | async (joint)
0.074      1.3962264150943395 % bnet/n3s1c1a.bnet | async (disjoint)
18.975     1.2923108356602875 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
420.506    1.4165176060015023 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.689      1.2806691449814125 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2407.238   1.582260193296665  % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2.37       1.403197158081705  % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
13479.298  1.5852602167285887 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
4.188      1.2516437537358038 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
6.161      1.4034168564920273 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
51.626     1.4976647036639494 % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
644.269    4.54017504791972   % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
4159.577   1.5761251115903963 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2027.243   1.221433804656678  % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
40933.506  1.6872223617243298 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
55999.634  1.786259111974617  % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
6308.131   1.3306207486885495 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
2.644      1.2878714076960547 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
519.891    1.490167134352401  % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.397      1.2563291139240507 % bnet/n6s1c2.bnet | async (joint)
17.555     1.2646783372955839 % bnet/faure_cellcycle.bnet | async (joint)
0.579      1.5117493472584855 % bnet/n5s3.bnet | async (disjoint)
20178.386  1.297327202189765  % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
3.821      1.277072192513369  % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
22.566     1.5012973188743262 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
771.909    1.2917271189248618 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
3251.146   1.3252236494718705 % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.216      1.2934131736526946 % bnet/raf.bnet | async (joint)
3391.882   1.322973064158235  % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
155.056    1.8162607911351631 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
4167.131   1.5945680777276798 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2703.455   1.6068789949751134 % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
15637.631  1.6563764052203673 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
77.479     1.2124849376379085 % bnet/tournier_apoptosis.bnet | async (joint)
9.383      1.2869290906597173 % bnet/arellano_rootstem.bnet | async (joint)
837.529    1.5662945092758827 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)


==> data/scc.adiar-skip_transpose.tex <==
101.424    1.19492453963878   % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
2.473      1.1074787281683833 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
27985.073  1.2004393978507022 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
2331.835   1.1924482818222635 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
4084.048   1.172894845067122  % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
91.88      1.1695965986481154 % bnet/faure_cellcycle.bnet | async (disjoint)
0.736      1.130568356374808  % bnet/n7s3.bnet | async (joint)
6.046      1.1638113570741098 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
27822.061  1.2919053867813788 % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
337.706    1.8898035243621956 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
173.02     1.2059664041262983 % bnet/saadatpour_guardcell.bnet | async (disjoint)
374.743    1.2090550965165012 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
6431.27    1.1869994776757122 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
265.491    3.517508645017687  % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
34.3       1.3181154407808777 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
1.315      1.1545215100965758 % bnet/n6s1c2.bnet | async (disjoint)
2216.942   1.1895495046901778 % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
6303.276   1.1672943013976362 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
14276.38   1.8241619121655428 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
59.932     1.484273614344445  % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
2853.436   1.239890656007467  % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
785.574    1.1416866013062397 % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
782.452    1.272058357326449  % aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
93.326     1.1615512906678613 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
1276.115   1.181440282927597  % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
0.107      1.1758241758241759 % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
26.46      1.1960403200289291 % bnet/saadatpour_guardcell.bnet | async (joint)
106212.906 1.2483210946130747 % aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
19.097     1.063425771244014  % bnet/xiao_wnt5a.bnet | async (disjoint)
0.868      1.2579710144927536 % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.123      1.123              % bnet/multivalued.bnet | async (joint)
75240.404  1.2973832055749381 % aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
30.005     1.1698311825022418 % bnet/n12c5.bnet | async (joint)
378.681    1.1461497484821153 % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.542      1.097165991902834  % bnet/raf.bnet | async (disjoint)
9649.283   1.5004080169103107 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
4.716      1.1086036671368125 % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
7539.366   1.23303893279847   % aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
173.719    1.1954403446235151 % bnet/dinwoodie_stomatal.bnet | async (disjoint)
4837.777   1.3367108158926162 % mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.232      1.0841121495327104 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
9.495      1.1210153482880754 % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
11884.195  1.253534209140376  % bnet/dinwoodie_life.bnet | async (disjoint)
17.139     1.1696580904934142 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
823.633    1.141991750147319  % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
10291.597  1.220147424050792  % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
48270.546  1.872445505256462  % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
0.334      1.2234432234432233 % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
10.405     1.1515050907481186 % aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
3270.277   1.1961304981223806 % aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
17.241     1.149553273769836  % bnet/davidich_yeast.bnet | async (joint)
1435.649   1.0087252174805073 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.286      1.144              % aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
770.567    1.2673424142048426 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
1148.263   1.9369570424649722 % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
10.04      2.9017341040462425 % aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
2.605      1.1104006820119352 % bnet/n7s3.bnet | async (disjoint)
2752.069   1.4241132762632867 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.039      1.1470588235294117 % bnet/n3s1c1a.bnet | async (joint)
22.831     1.270860005566379  % mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
4140.611   1.1106115884605707 % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
16446.601  1.2310782529507633 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
481.022    1.1988206736017306 % bnet/tournier_apoptosis.bnet | async (disjoint)
98.276     1.1818127157064349 % aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
36.024     1.2104025267119145 % bnet/randomnet_n15k3.bnet | async (disjoint)
80.338     1.1662626115990418 % aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
82.426     1.1631904264627022 % bnet/davidich_yeast.bnet | async (disjoint)
218.442    1.5069642302783621 % mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
65178.081  1.3375015236638852 % aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
4.707      1.48251968503937   % mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
211.962    0.9348405193705455 % mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
4.654      1.1190189949507094 % bnet/xiao_wnt5a.bnet | async (joint)
168.787    1.1929421576388104 % bnet/n12c5.bnet | async (disjoint)
604.915    1.8992621664050235 % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
1575.205   1.1774645423734893 % aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
1537.788   1.1964838133414666 % bnet/dinwoodie_life.bnet | async (joint)
0.259      1.1511111111111112 % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.837      1.1403269754768393 % aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
2249.329   1.3686670378381998 % mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
1947.618   1.210305774005015  % aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
1052.287   1.1817169077557659 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
175.68     1.2418092753991985 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.077      1.0845070422535212 % bnet/n3s1c1b.bnet | async (disjoint)
15.612     1.0087878004652364 % mcc/2023/Anderson/anderson_04.pnml | async (joint)
0.511      1.148314606741573  % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
1.639      1.1126951799049558 % bnet/randomnet_n7k3.bnet | async (joint)
141.604    1.1679258355052622 % aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
17907.949  1.267887258249008  % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
19.976     1.1550826876373308 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
3.76       1.1820182332599811 % bnet/multivalued.bnet | async (disjoint)
6.4        1.1247803163444638 % bnet/randomnet_n7k3.bnet | async (disjoint)
4243.465   1.2400413788871243 % aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
4.174      1.1354733405875952 % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
6.28       1.1808950733358408 % bnet/randomnet_n15k3.bnet | async (joint)
17.11      1.0982028241335045 % aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
25.603     1.1650967007963595 % bnet/dinwoodie_stomatal.bnet | async (joint)
1.366      0.38478873239436623 % aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
34823.789  1.2364804491351418 % aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
355.76     1.1389422461262644 % aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
18160.492  1.224248551856341  % aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
19.315     1.1164094561008036 % aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
40.358     1.214395329943129  % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
44.156     1.031923346576303  % mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
23.536     1.406057709540594  % mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
126.005    3.2011838829327774 % bnet/arellano_rootstem.bnet | async (disjoint)
0.042      1.105263157894737  % bnet/n3s1c1b.bnet | async (joint)
0.192      1.0971428571428572 % bnet/n5s3.bnet | async (joint)
0.074      1.121212121212121  % bnet/n3s1c1a.bnet | async (disjoint)
18.975     1.1253780914536504 % aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
420.506    1.3197272079615605 % mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
0.689      1.0936507936507935 % aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2407.238   1.3012941379981402 % aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2.37       1.1544081831466149 % aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
13479.298  1.3049162375369412 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
4.188      1.1267150928167877 % aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
6.161      1.2822060353798126 % mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
51.626     1.1660041557502934 % aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
644.269    3.6011995260027727 % aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
4159.577   1.225415763100688  % aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2027.243   1.1788476008936535 % aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
40933.506  1.2523707415813736 % aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
55999.634  1.3207668932142609 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
6308.131   1.2194766952945184 % aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
2.644      1.2384074941451992 % mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
519.891    1.4486929771030652 % mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.397      1.1375358166189113 % bnet/n6s1c2.bnet | async (joint)
17.555     1.1285760205721633 % bnet/faure_cellcycle.bnet | async (joint)
0.579      1.1442687747035571 % bnet/n5s3.bnet | async (disjoint)
20178.386  1.3677947108069035 % mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
3.821      1.1392367322599881 % aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
22.566     1.122686567164179  % aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
771.909    1.2590098318730143 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
3251.146   1.178038094830888  % aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
0.216      1.0964467005076142 % bnet/raf.bnet | async (joint)
3391.882   1.1752304633659745 % aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
155.056    1.8053699089490722 % mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
4167.131   1.2525281216335795 % aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
2703.455   1.2174582866674504 % aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
15637.631  1.2399462904566998 % aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
77.479     1.0885398373069952 % bnet/tournier_apoptosis.bnet | async (joint)
9.383      1.126005040201608  % bnet/arellano_rootstem.bnet | async (joint)
837.529    1.1949626399841342 % aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)


==> data/scc.buddy.tex <==
0.001      0.538      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.186      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.205      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.084      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.585      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.205      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.016      15.031     %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.008      3.661      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.006      1.689      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.002      0.41       %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.009      4.062      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.004      1.067      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.012      6.863      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.006      1.983      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.029      34.471     %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.013      7.332      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.017      11.217     %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.009      2.992      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.022      12.124     %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.011      3.267      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.022      13.429     %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.01       3.346      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.055      59.579     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.026      14.683     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.053      60.2       %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.026      14.798     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.098      141.904    %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.04       79.137     %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.434      534.72     %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.176      134.756    %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.228      242.807    %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.099      61.784     %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.03       3.438      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.021      0.714      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.403      1521.392   %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.401      295.896    %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
1.379      1450.176   %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.393      273.86     %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.743      663.08     %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.219      109.031    %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
1.452      1682.426   %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.425      287.459    %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
1.79       2639.116   %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.578      618.835    %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
1.835      2613.329   %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.578      597.579    %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
2.132      2662.298   %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.731      647.525    %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
1.722      1283.5     %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.635      279.762    %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
5.424      6390.939   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
1.442      1189.284   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
4.791      4789.427   %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
1.485      977.78     %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
6.911      9440.868   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
2.392      2173.049   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
7.108      10124.511  %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
2.51       2563.833   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
12.292     10943.434  %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
2.353      1671.01    %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.492      478.474    %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.137      77.491     %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.548      475.727    %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.158      75.595     %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
8.641      8502.893   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
2.521      1659.724   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
9.189      10914.827  %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
2.841      2453.281   %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
10.629     15740.391  %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
2.845      2473.49    %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
17.602     24260.884  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
4.555      11961.318  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
18.76      20534.124  %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
4.151      3152.218   %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
19.318     34081.388  %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
5.88       4831.251   %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
32.063     31350.23   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
7.732      4740.743   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
44.876     64303.351  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
20.235     21449.051  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
44.026     44199.03   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
10.302     6889.622   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.029      28.919     %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.012      7.291      %                    bnet/arellano_rootstem.bnet | async (joint)
0.055      51.217     %                    bnet/davidich_yeast.bnet | async (disjoint)
0.023      13.284     %                    bnet/davidich_yeast.bnet | async (joint)
5.593      7157.849   %                    bnet/dinwoodie_life.bnet | async (disjoint)
1.415      1217.64    %                    bnet/dinwoodie_life.bnet | async (joint)
0.132      113.395    %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.048      19.964     %                    bnet/dinwoodie_stomatal.bnet | async (joint)
0.064      60.91      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.027      13.881     %                    bnet/faure_cellcycle.bnet | async (joint)
0.008      2.409      %                    bnet/multivalued.bnet | async (disjoint)
0.004      0.882      %                    bnet/multivalued.bnet | async (joint)
0.106      111.444    %                    bnet/n12c5.bnet | async (disjoint)
0.038      23.436     %                    bnet/n12c5.bnet | async (joint)
0.001      0.053      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.03       %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.056      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.034      %                    bnet/n3s1c1b.bnet | async (joint)
0.001      0.383      %                    bnet/n5s3.bnet | async (disjoint)
0.001      0.152      %                    bnet/n5s3.bnet | async (joint)
0.001      0.906      %                    bnet/n6s1c2.bnet | async (disjoint)
0.001      0.316      %                    bnet/n6s1c2.bnet | async (joint)
0.003      1.837      %                    bnet/n7s3.bnet | async (disjoint)
0.001      0.58       %                    bnet/n7s3.bnet | async (joint)
0.001      0.366      %                    bnet/raf.bnet | async (disjoint)
0.001      0.167      %                    bnet/raf.bnet | async (joint)
0.081      23.437     %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.045      4.885      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.008      4.515      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.004      1.318      %                    bnet/randomnet_n7k3.bnet | async (joint)
0.132      112.067    %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.048      19.882     %                    bnet/saadatpour_guardcell.bnet | async (joint)
0.262      310.593    %                    bnet/tournier_apoptosis.bnet | async (disjoint)
0.084      63.901     %                    bnet/tournier_apoptosis.bnet | async (joint)
0.014      13.357     %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.007      3.649      %                    bnet/xiao_wnt5a.bnet | async (joint)
1.131      85.371     %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.202      14.395     %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
1.944      203.418    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.569      40.586     %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
60.043     3399.353   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
15.499     1351.238   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)
0.023      16.481     %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.009      2.053      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.315      348.881    %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.072      24.504     %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
4.758      6013.969   %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.719      296.859    %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
70.959     106306.715 %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
7.241      3466.959   %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
1.109      628.17     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.135      14.828     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
13.273     7198.98    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
1.309      149.153    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
1615.96    200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
121.111    15553.814  %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
1212.002   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
%.???      172800.0   %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.006      3.226      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.257      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
2.468      1747.666   %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.402      240.216    %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.06       38.909     %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.021      4.39       %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
31.09      25150.276  %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
5.777      1535.041   %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)


==> data/scc.cal.tex <==
0.165      6.863      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.07       1.983      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.655      34.471     %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.269      7.332      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.296      11.217     %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.113      2.992      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.363      12.124     %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.123      3.267      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.378      13.429     %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.118      3.346      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.653      59.579     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.611      14.683     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
1.654      60.2       %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.606      14.798     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
3.005      141.904    %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
1.165      79.137     %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
14.196     534.72     %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
4.663      134.756    %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
6.635      242.807    %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
2.131      61.784     %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.131      3.438      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.03       0.714      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
47.844     1521.392   %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
11.026     295.896    %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
47.809     1450.176   %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
11.033     273.86     %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
21.852     663.08     %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
4.657      109.031    %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
51.038     1682.426   %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
10.51      287.459    %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
58.013     2639.116   %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
19.525     618.835    %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
65.069     2613.329   %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
20.959     597.579    %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
55.676     2662.298   %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
19.014     647.525    %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
39.672     1283.5     %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
10.555     279.762    %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
209.709    6390.939   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
46.259     1189.284   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
147.013    4789.427   %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
34.387     977.78     %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
318.083    9440.868   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
94.294     2173.049   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
268.316    10124.511  %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
84.658     2563.833   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
437.385    10943.434  %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
79.273     1671.01    %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
20.226     478.474    %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
3.052      77.491     %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
20.346     475.727    %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
3.103      75.595     %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
272.213    8502.893   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
59.526     1659.724   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
327.555    10914.827  %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
84.818     2453.281   %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
402.769    15740.391  %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
84.777     2473.49    %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
784.239    24260.884  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
187.159    11961.318  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
721.792    20534.124  %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
121.678    3152.218   %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
700.145    34081.388  %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
161.217    4831.251   %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
1104.97    31350.23   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
183.743    4740.743   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
1455.802   64303.351  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
699.236    21449.051  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
1746.786   44199.03   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
255.04     6889.622   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.009      0.538      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.006      0.186      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.006      0.205      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.003      0.084      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.018      0.585      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.008      0.205      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.381      15.031     %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.142      3.661      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.044      1.689      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.014      0.41       %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.103      4.062      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.036      1.067      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.673      28.919     %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.279      7.291      %                    bnet/arellano_rootstem.bnet | async (joint)
1.447      51.217     %                    bnet/davidich_yeast.bnet | async (disjoint)
0.471      13.284     %                    bnet/davidich_yeast.bnet | async (joint)
230.714    7157.849   %                    bnet/dinwoodie_life.bnet | async (disjoint)
43.752     1217.64    %                    bnet/dinwoodie_life.bnet | async (joint)
4.01       113.395    %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.832      19.964     %                    bnet/dinwoodie_stomatal.bnet | async (joint)
1.758      60.91      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.529      13.881     %                    bnet/faure_cellcycle.bnet | async (joint)
0.071      2.409      %                    bnet/multivalued.bnet | async (disjoint)
0.038      0.882      %                    bnet/multivalued.bnet | async (joint)
3.316      111.444    %                    bnet/n12c5.bnet | async (disjoint)
0.858      23.436     %                    bnet/n12c5.bnet | async (joint)
0.001      0.053      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.03       %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.056      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.034      %                    bnet/n3s1c1b.bnet | async (joint)
0.009      0.383      %                    bnet/n5s3.bnet | async (disjoint)
0.006      0.152      %                    bnet/n5s3.bnet | async (joint)
0.021      0.906      %                    bnet/n6s1c2.bnet | async (disjoint)
0.011      0.316      %                    bnet/n6s1c2.bnet | async (joint)
0.043      1.837      %                    bnet/n7s3.bnet | async (disjoint)
0.019      0.58       %                    bnet/n7s3.bnet | async (joint)
0.008      0.366      %                    bnet/raf.bnet | async (disjoint)
0.006      0.167      %                    bnet/raf.bnet | async (joint)
0.882      23.437     %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.26       4.885      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.124      4.515      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.044      1.318      %                    bnet/randomnet_n7k3.bnet | async (joint)
4.013      112.067    %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.806      19.882     %                    bnet/saadatpour_guardcell.bnet | async (joint)
9.14       310.593    %                    bnet/tournier_apoptosis.bnet | async (disjoint)
2.247      63.901     %                    bnet/tournier_apoptosis.bnet | async (joint)
0.255      13.357     %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.136      3.649      %                    bnet/xiao_wnt5a.bnet | async (joint)
0.505      38.909     %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.202      4.39       %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
242.54     25150.276  %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
74.456     1535.041   %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.132      16.481     %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.069      2.053      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
2.217      348.881    %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.877      24.504     %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
34.234     6013.969   %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
10.778     296.859    %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
451.74     106306.715 %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
159.181    3466.959   %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
2.438      628.17     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.733      14.828     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
28.8       7198.98    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
7.097      149.153    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
3448.232   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
1899.633   15553.814  %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
39695.01   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
%.???      200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.027      3.226      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.006      0.257      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
20.78      1747.666   %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
36.548     240.216    %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
4.851      85.371     %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
1.6        14.395     %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
11.065     203.418    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
16.437     40.586     %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
6559.103   3399.353   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
1153.485   1351.238   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)


==> data/scc.cudd.tex <==
0.011      6.863      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.003      1.983      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.056      34.471     %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.012      7.332      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.024      11.217     %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.007      2.992      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.028      12.124     %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.008      3.267      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.028      13.429     %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.008      3.346      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.129      59.579     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.034      14.683     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.128      60.2       %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.034      14.798     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.266      141.904    %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.063      79.137     %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
1.168      534.72     %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.312      134.756    %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.526      242.807    %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.143      61.784     %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.036      3.438      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.013      0.714      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
3.798      1521.392   %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.791      295.896    %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
3.804      1450.176   %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.76       273.86     %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
1.771      663.08     %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.366      109.031    %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
4.119      1682.426   %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.797      287.459    %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
5.174      2639.116   %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
1.175      618.835    %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
5.22       2613.329   %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
1.279      597.579    %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
5.304      2662.298   %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
1.416      647.525    %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
3.688      1283.5     %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
1.031      279.762    %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
17.113     6390.939   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
3.53       1189.284   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
12.667     4789.427   %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
2.956      977.78     %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
24.936     9440.868   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
6.382      2173.049   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
20.503     10124.511  %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
5.459      2563.833   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
33.146     10943.434  %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
5.102      1671.01    %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
1.746      478.474    %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.28       77.491     %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
1.821      475.727    %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.311      75.595     %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
23.599     8502.893   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
5.284      1659.724   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
27.281     10914.827  %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
6.265      2453.281   %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
34.874     15740.391  %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
6.179      2473.49    %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
56.642     24260.884  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
11.497     11961.318  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
55.153     20534.124  %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
9.168      3152.218   %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
64.246     34081.388  %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
11.62      4831.251   %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
94.506     31350.23   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
15.377     4740.743   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
133.087    64303.351  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
52.442     21449.051  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
170.094    44199.03   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
30.939     6889.622   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.538      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.186      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.205      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.084      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.585      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.205      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.029      15.031     %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.007      3.661      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.003      1.689      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.41       %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.008      4.062      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.002      1.067      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.057      28.919     %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.013      7.291      %                    bnet/arellano_rootstem.bnet | async (joint)
0.12       51.217     %                    bnet/davidich_yeast.bnet | async (disjoint)
0.029      13.284     %                    bnet/davidich_yeast.bnet | async (joint)
17.985     7157.849   %                    bnet/dinwoodie_life.bnet | async (disjoint)
3.293      1217.64    %                    bnet/dinwoodie_life.bnet | async (joint)
0.332      113.395    %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.071      19.964     %                    bnet/dinwoodie_stomatal.bnet | async (joint)
0.142      60.91      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.036      13.881     %                    bnet/faure_cellcycle.bnet | async (joint)
0.005      2.409      %                    bnet/multivalued.bnet | async (disjoint)
0.001      0.882      %                    bnet/multivalued.bnet | async (joint)
0.247      111.444    %                    bnet/n12c5.bnet | async (disjoint)
0.055      23.436     %                    bnet/n12c5.bnet | async (joint)
0.001      0.053      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.03       %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.056      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.034      %                    bnet/n3s1c1b.bnet | async (joint)
0.001      0.383      %                    bnet/n5s3.bnet | async (disjoint)
0.001      0.152      %                    bnet/n5s3.bnet | async (joint)
0.001      0.906      %                    bnet/n6s1c2.bnet | async (disjoint)
0.001      0.316      %                    bnet/n6s1c2.bnet | async (joint)
0.003      1.837      %                    bnet/n7s3.bnet | async (disjoint)
0.001      0.58       %                    bnet/n7s3.bnet | async (joint)
0.001      0.366      %                    bnet/raf.bnet | async (disjoint)
0.001      0.167      %                    bnet/raf.bnet | async (joint)
0.282      23.437     %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.081      4.885      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.009      4.515      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.002      1.318      %                    bnet/randomnet_n7k3.bnet | async (joint)
0.333      112.067    %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.072      19.882     %                    bnet/saadatpour_guardcell.bnet | async (joint)
0.763      310.593    %                    bnet/tournier_apoptosis.bnet | async (disjoint)
0.171      63.901     %                    bnet/tournier_apoptosis.bnet | async (joint)
0.022      13.357     %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.006      3.649      %                    bnet/xiao_wnt5a.bnet | async (joint)
0.096      38.909     %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.027      4.39       %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
66.367     25150.276  %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
12.863     1535.041   %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.029      16.481     %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.006      2.053      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.622      348.881    %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.096      24.504     %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
11.589     6013.969   %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
1.255      296.859    %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
206.107    106306.715 %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
18.814     3466.959   %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
1.428      628.17     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.112      14.828     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
18.441     7198.98    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
1.171      149.153    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
3721.999   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
145.643    15553.814  %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
1319.913   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
11632.707  200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.007      3.226      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.257      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
9.829      1747.666   %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.799      240.216    %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
4.294      85.371     %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.342      14.395     %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
7.107      203.418    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
1.15       40.586     %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
276.679    3399.353   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
43.212     1351.238   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)


==> data/scc.libbdd.tex <==
0.048      6.863      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.015      1.983      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.221      34.471     %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.052      7.332      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.077      11.217     %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.022      2.992      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.088      12.124     %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.027      3.267      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.096      13.429     %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.026      3.346      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.44       59.579     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.117      14.683     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.44       60.2       %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.116      14.798     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
1.122      141.904    %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.249      79.137     %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
4.733      534.72     %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
1.269      134.756    %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
2.028      242.807    %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.571      61.784     %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.078      3.438      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.044      0.714      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
14.712     1521.392   %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
2.857      295.896    %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
14.346     1450.176   %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
2.726      273.86     %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
6.395      663.08     %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
1.214      109.031    %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
17.607     1682.426   %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
3.317      287.459    %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
24.262     2639.116   %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
5.42       618.835    %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
25.024     2613.329   %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
5.857      597.579    %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
25.249     2662.298   %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
5.433      647.525    %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
13.091     1283.5     %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
3.109      279.762    %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
59.194     6390.939   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
12.997     1189.284   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
50.808     4789.427   %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
10.181     977.78     %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
97.93      9440.868   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
22.243     2173.049   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
93.9       10124.511  %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
27.466     2563.833   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
131.174    10943.434  %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
19.878     1671.01    %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
6.126      478.474    %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
1.213      77.491     %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
6.091      475.727    %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
1.21       75.595     %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
90.472     8502.893   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
18.998     1659.724   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
115.19     10914.827  %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
25.909     2453.281   %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
171.872    15740.391  %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
23.726     2473.49    %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
235.996    24260.884  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
54.283     11961.318  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
235.792    20534.124  %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
38.027     3152.218   %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
374.954    34081.388  %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
53.508     4831.251   %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
366.048    31350.23   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
60.069     4740.743   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
673.898    64303.351  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
240.006    21449.051  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
609.896    44199.03   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
107.816    6889.622   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.538      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.186      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.205      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.084      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.002      0.585      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.205      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.094      15.031     %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.024      3.661      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.012      1.689      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.003      0.41       %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.027      4.062      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.009      1.067      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.215      28.919     %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.056      7.291      %                    bnet/arellano_rootstem.bnet | async (joint)
0.421      51.217     %                    bnet/davidich_yeast.bnet | async (disjoint)
0.11       13.284     %                    bnet/davidich_yeast.bnet | async (joint)
76.282     7157.849   %                    bnet/dinwoodie_life.bnet | async (disjoint)
13.879     1217.64    %                    bnet/dinwoodie_life.bnet | async (joint)
1.195      113.395    %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.262      19.964     %                    bnet/dinwoodie_stomatal.bnet | async (joint)
0.485      60.91      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.121      13.881     %                    bnet/faure_cellcycle.bnet | async (joint)
0.02       2.409      %                    bnet/multivalued.bnet | async (disjoint)
0.007      0.882      %                    bnet/multivalued.bnet | async (joint)
0.846      111.444    %                    bnet/n12c5.bnet | async (disjoint)
0.187      23.436     %                    bnet/n12c5.bnet | async (joint)
0.001      0.053      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.03       %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.056      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.034      %                    bnet/n3s1c1b.bnet | async (joint)
0.001      0.383      %                    bnet/n5s3.bnet | async (disjoint)
0.001      0.152      %                    bnet/n5s3.bnet | async (joint)
0.003      0.906      %                    bnet/n6s1c2.bnet | async (disjoint)
0.001      0.316      %                    bnet/n6s1c2.bnet | async (joint)
0.009      1.837      %                    bnet/n7s3.bnet | async (disjoint)
0.003      0.58       %                    bnet/n7s3.bnet | async (joint)
0.001      0.366      %                    bnet/raf.bnet | async (disjoint)
0.001      0.167      %                    bnet/raf.bnet | async (joint)
0.645      23.437     %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.251      4.885      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.029      4.515      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.01       1.318      %                    bnet/randomnet_n7k3.bnet | async (joint)
1.187      112.067    %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.262      19.882     %                    bnet/saadatpour_guardcell.bnet | async (joint)
2.779      310.593    %                    bnet/tournier_apoptosis.bnet | async (disjoint)
0.654      63.901     %                    bnet/tournier_apoptosis.bnet | async (joint)
0.083      13.357     %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.023      3.649      %                    bnet/xiao_wnt5a.bnet | async (joint)
0.345      38.909     %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.084      4.39       %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
214.445    25150.276  %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
33.555     1535.041   %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.148      16.481     %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.031      2.053      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
3.472      348.881    %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.469      24.504     %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
70.45      6013.969   %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
6.352      296.859    %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
1247.742   106306.715 %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
79.018     3466.959   %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
6.516      628.17     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.565      14.828     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
98.239     7198.98    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
6.074      149.153    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
24251.237  200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
2524.387   15553.814  %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.002      0.001      %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
113601.637 200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.005      0.001      %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
200000     200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.031      3.226      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.005      0.257      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
52.253     1747.666   %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
270.236    240.216    %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
8.508      85.371     %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
1.788      14.395     %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
18.002     203.418    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
4.925      40.586     %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
853.852    3399.353   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
380.811    1351.238   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)


==> data/scc.sylvan.tex <==
0.004      6.863      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (disjoint)
0.001      1.983      %                    aeon/[v10]__[r14]__[AP-1-ELSE-0-WT]__[ginsim].aeon | async (joint)
0.017      34.471     %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (disjoint)
0.005      7.332      %                    aeon/[v10]__[r18]__[ROOT-STEM-CELL-NICHE]__[biomodels].aeon | async (joint)
0.008      11.217     %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (disjoint)
0.004      2.992      %                    aeon/[v10]__[r27]__[FISSION-YEAST-DAVIDICH-2008]__[ginsim].aeon | async (joint)
0.009      12.124     %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (disjoint)
0.004      3.267      %                    aeon/[v10]__[r34]__[BOOLEAN-CELL-CYCLE]__[ginsim].aeon | async (joint)
0.01       13.429     %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.004      3.346      %                    aeon/[v10]__[r35]__[MAMMALIAN-CELL-CYCLE]__[cellcollective].aeon | async (joint)
0.04       59.579     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
0.015      14.683     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
0.038      60.2       %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
0.015      14.798     %                    aeon/[v11]__[r11]__[TOLL-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
0.074      141.904    %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (disjoint)
0.025      79.137     %                    aeon/[v12]__[r30]__[METABOLIC-INTERACTIONS-IN-THE-GUT-MICROBIOME]__[cellcollective].aeon | async (joint)
0.325      534.72     %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (disjoint)
0.138      134.756    %                    aeon/[v13]__[r18]__[REGULATION-OF-THE-LARABINOSE-OPERON]__[cellcollective].aeon | async (joint)
0.172      242.807    %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (disjoint)
0.071      61.784     %                    aeon/[v13]__[r22]__[LAC-OPERON]__[cellcollective].aeon | async (joint)
0.015      3.438      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.01       0.714      %                    aeon/[v14]__[r66]__[ARABIDOPSIS-THALIANA-CELL-CYCLE]__[cellcollective].aeon | async (joint)
1.328      1521.392   %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.384      295.896    %                    aeon/[v15]__[r38]__[CARDIAC-DEVELOPMENT]__[cellcollective].aeon | async (joint)
1.413      1450.176   %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (disjoint)
0.377      273.86     %                    aeon/[v15]__[r38]__[PREDICTING-VARIABLES-IN-CARDIAC-GENE]__[cellcollective].aeon | async (joint)
0.598      663.08     %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (disjoint)
0.179      109.031    %                    aeon/[v15]__[r66]__[FANCONI-ANEMIA-AND-CHECKPOINT-RECOVERY]__[cellcollective].aeon | async (joint)
1.354      1682.426   %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (disjoint)
0.359      287.459    %                    aeon/[v16]__[r22]__[NEUROTRANSMITTER-SIGNALING-PATHWAY]__[cellcollective].aeon | async (joint)
1.688      2639.116   %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.534      618.835    %                    aeon/[v16]__[r41]__[SKBR3-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
1.683      2613.329   %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.541      597.579    %                    aeon/[v16]__[r46]__[BT474-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
1.632      2662.298   %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (disjoint)
0.613      647.525    %                    aeon/[v16]__[r46]__[HCC1954-BREAST-CELL-LINE]__[cellcollective].aeon | async (joint)
1.444      1283.5     %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (disjoint)
0.524      279.762    %                    aeon/[v16]__[r58]__[MAPK-RED3-19-06-2013]__[ginsim].aeon | async (joint)
6.96       6390.939   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (disjoint)
1.729      1189.284   %                    aeon/[v17]__[r29]__[DROSOPHILA-BODY-SEGMENTATION]__[cellcollective].aeon | async (joint)
5.084      4789.427   %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (disjoint)
1.393      977.78     %                    aeon/[v17]__[r78]__[MAPK-RED1-19-06-2013]__[ginsim].aeon | async (joint)
7.957      9440.868   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (disjoint)
2.489      2173.049   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-12-06-2013]__[ginsim].aeon | async (joint)
7.526      10124.511  %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (disjoint)
2.602      2563.833   %                    aeon/[v18]__[r18]__[VEGF-PATHWAY-OF-DROSOPHILA]__[cellcollective].aeon | async (joint)
14.677     10943.434  %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (disjoint)
2.531      1671.01    %                    aeon/[v18]__[r43]__[TLGL-SURVIVAL-NETWORK]__[cellcollective].aeon | async (joint)
0.473      478.474    %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (disjoint)
0.134      77.491     %                    aeon/[v18]__[r58]__[BUDDING-YEAST-IRONS-2009]__[ginsim].aeon | async (joint)
0.51       475.727    %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (disjoint)
0.156      75.595     %                    aeon/[v18]__[r59]__[BUDDING-YEAST-CELL-CYCLE]__[cellcollective].aeon | async (joint)
10.161     8502.893   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (disjoint)
2.661      1659.724   %                    aeon/[v18]__[r60]__[MAPK-RED2-12-06-2013]__[ginsim].aeon | async (joint)
13.087     10914.827  %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (disjoint)
3.457      2453.281   %                    aeon/[v18]__[r78]__[CD4-T-CELL-DIFFERENTIATION]__[cellcollective].aeon | async (joint)
15.722     15740.391  %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (disjoint)
3.43       2473.49    %                    aeon/[v18]__[r83]__[T-CD4-LYMPHOCYTE-TRANSCRIPTION]__[biomodels].aeon | async (joint)
22.29      24260.884  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (disjoint)
5.927      11961.318  %                    aeon/[v19]__[r21]__[JNK-PATHWAY]__[covid-uni-lu].aeon | async (joint)
25.402     20534.124  %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (disjoint)
5.276      3152.218   %                    aeon/[v19]__[r32]__[OXIDATIVE-STRESS-PATHWAY]__[cellcollective].aeon | async (joint)
26.865     34081.388  %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (disjoint)
6.708      4831.251   %                    aeon/[v19]__[r73]__[INFLAMMATORY-RESPONSES]__[biomodels].aeon | async (joint)
48.527     31350.23   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (disjoint)
9.76       4740.743   %                    aeon/[v19]__[r79]__[HUMAN-GONADAL-SEX-DETERMINATION]__[cellcollective].aeon | async (joint)
56.181     64303.351  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (disjoint)
26.478     21449.051  %                    aeon/[v21]__[r24]__[TGFB-pathway]__[covid-uni-lu].aeon | async (joint)
62.051     44199.03   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (disjoint)
14.248     6889.622   %                    aeon/[v23]__[r43]__[AURORA-KINASE-A-IN-NEUROBLASTOMA]__[cellcollective].aeon | async (joint)
0.001      0.538      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (disjoint)
0.001      0.186      %                    aeon/[v5]__[r14]__[CORTICAL-AREA-DEVELOPMENT]__[cellcollective].aeon | async (joint)
0.001      0.205      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (disjoint)
0.001      0.084      %                    aeon/[v5]__[r15]__[G2A]__[ginsim].aeon | async (joint)
0.001      0.585      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (disjoint)
0.001      0.205      %                    aeon/[v6]__[r11]__[ZEBRA-MIR9-22-07-2011]__[ginsim].aeon | async (joint)
0.008      15.031     %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (disjoint)
0.003      3.661      %                    aeon/[v9]__[r12]__[G2B]__[ginsim].aeon | async (joint)
0.001      1.689      %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (disjoint)
0.001      0.41       %                    aeon/[v9]__[r19]__[BUDDING-YEAST-ORLANDO-2008]__[ginsim].aeon | async (joint)
0.002      4.062      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (disjoint)
0.001      1.067      %                    aeon/[v9]__[r19]__[CELL-CYCLE-TRANSCRIPTION]__[cellcollective].aeon | async (joint)
0.017      28.919     %                    bnet/arellano_rootstem.bnet | async (disjoint)
0.005      7.291      %                    bnet/arellano_rootstem.bnet | async (joint)
0.038      51.217     %                    bnet/davidich_yeast.bnet | async (disjoint)
0.014      13.284     %                    bnet/davidich_yeast.bnet | async (joint)
6.665      7157.849   %                    bnet/dinwoodie_life.bnet | async (disjoint)
1.497      1217.64    %                    bnet/dinwoodie_life.bnet | async (joint)
0.116      113.395    %                    bnet/dinwoodie_stomatal.bnet | async (disjoint)
0.041      19.964     %                    bnet/dinwoodie_stomatal.bnet | async (joint)
0.047      60.91      %                    bnet/faure_cellcycle.bnet | async (disjoint)
0.016      13.881     %                    bnet/faure_cellcycle.bnet | async (joint)
0.002      2.409      %                    bnet/multivalued.bnet | async (disjoint)
0.001      0.882      %                    bnet/multivalued.bnet | async (joint)
0.085      111.444    %                    bnet/n12c5.bnet | async (disjoint)
0.025      23.436     %                    bnet/n12c5.bnet | async (joint)
0.001      0.053      %                    bnet/n3s1c1a.bnet | async (disjoint)
0.001      0.03       %                    bnet/n3s1c1a.bnet | async (joint)
0.001      0.056      %                    bnet/n3s1c1b.bnet | async (disjoint)
0.001      0.034      %                    bnet/n3s1c1b.bnet | async (joint)
0.001      0.383      %                    bnet/n5s3.bnet | async (disjoint)
0.001      0.152      %                    bnet/n5s3.bnet | async (joint)
0.001      0.906      %                    bnet/n6s1c2.bnet | async (disjoint)
0.001      0.316      %                    bnet/n6s1c2.bnet | async (joint)
0.001      1.837      %                    bnet/n7s3.bnet | async (disjoint)
0.001      0.58       %                    bnet/n7s3.bnet | async (joint)
0.001      0.366      %                    bnet/raf.bnet | async (disjoint)
0.001      0.167      %                    bnet/raf.bnet | async (joint)
0.107      23.437     %                    bnet/randomnet_n15k3.bnet | async (disjoint)
0.062      4.885      %                    bnet/randomnet_n15k3.bnet | async (joint)
0.002      4.515      %                    bnet/randomnet_n7k3.bnet | async (disjoint)
0.001      1.318      %                    bnet/randomnet_n7k3.bnet | async (joint)
0.116      112.067    %                    bnet/saadatpour_guardcell.bnet | async (disjoint)
0.041      19.882     %                    bnet/saadatpour_guardcell.bnet | async (joint)
0.224      310.593    %                    bnet/tournier_apoptosis.bnet | async (disjoint)
0.08       63.901     %                    bnet/tournier_apoptosis.bnet | async (joint)
0.006      13.357     %                    bnet/xiao_wnt5a.bnet | async (disjoint)
0.002      3.649      %                    bnet/xiao_wnt5a.bnet | async (joint)
0.037      38.909     %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (disjoint)
0.017      4.39       %                    mcc/2021/GPUForwardProgress/gpufp_04_a.pnml | async (joint)
34.317     25150.276  %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (disjoint)
8.225      1535.041   %                    mcc/2021/GPUForwardProgress/gpufp_08_a.pnml | async (joint)
0.009      16.481     %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (disjoint)
0.003      2.053      %                    mcc/2022/AutonomousCar/autocar01_a.pnml | async (joint)
0.181      348.881    %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (disjoint)
0.054      24.504     %                    mcc/2022/AutonomousCar/autocar02_a.pnml | async (joint)
3.297      6013.969   %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (disjoint)
0.622      296.859    %                    mcc/2022/AutonomousCar/autocar03_a.pnml | async (joint)
69.324     106306.715 %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (disjoint)
9.158      3466.959   %                    mcc/2022/AutonomousCar/autocar04_a.pnml | async (joint)
0.455      628.17     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (disjoint)
0.101      14.828     %                    mcc/2022/StigmergyCommit/stigcomm02-a.pnml | async (joint)
6.959      7198.98    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (disjoint)
1.054      149.153    %                    mcc/2022/StigmergyCommit/stigcomm03-a.pnml | async (joint)
1471.989   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (disjoint)
153.989    15553.814  %                    mcc/2022/StigmergyCommit/stigcomm05-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (disjoint)
1547.244   200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm06-a.pnml | async (joint)
0.001      0.001      %                    mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (disjoint)
15947.485  200000     % ! NOTE ! TIMEOUT ! mcc/2022/StigmergyCommit/stigcomm07-a.pnml | async (joint)
0.002      3.226      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (disjoint)
0.001      0.257      %                    mcc/2022/StigmergyElection/stigelec02-a.pnml | async (joint)
1.761      1747.666   %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (disjoint)
0.748      240.216    %                    mcc/2022/StigmergyElection/stigelec06-a.pnml | async (joint)
0.924      85.371     %                    mcc/2023/Anderson/anderson_04.pnml | async (disjoint)
0.286      14.395     %                    mcc/2023/Anderson/anderson_04.pnml | async (joint)
1.582      203.418    %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (disjoint)
0.716      40.586     %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_03.pnml | async (joint)
88.282     3399.353   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (disjoint)
42.77      1351.238   %                    mcc/2023/EisenbergMcGuire/eisenberg-mcguire_04.pnml | async (joint)


